Drug-drug interaction prediction based on co-medication patterns and graph matching

Background: The problem of predicting whether a drug combination of arbitrary orders is likely to induce adverse drug reactions is considered in this manuscript. Methods: Novel kernels over drug combinations of arbitrary orders are developed within support vector machines for the prediction. Graph matching methods are used in the novel kernels to measure the similarities among drug combinations, in which drug co-medication patterns are leveraged to measure single drug similarities. Results: The experimental results on a real-world dataset demonstrated that the new kernels achieve an area under the curve (AUC) value 0.912 for the prediction problem. Conclusions: The new methods with drug co-medication based single drug similarities can accurately predict whether a drug combination is likely to induce adverse drug reactions of interest. Keywords: drug-drug interaction prediction; drug combination similarity; co-medication; graph matching

==> def.tex <==
\newcommand{\tran}{^{\mkern-1.5mu\mathsf{T}}}

% drugs
\newcommand{\drug}{\mbox{$\mathop{\mathtt{d}}\limits$}\xspace}
\newcommand{\drugi}{\mbox{$\mathop{\mathtt{d}_i}\limits$}\xspace}
\newcommand{\drugj}{\mbox{$\mathop{\mathtt{d}_j}\limits$}\xspace}
\newcommand{\D}{\mbox{$\mathop{D}\limits$}\xspace}
\newcommand{\Dp}{\mbox{$\mathop{D_p}\limits$}\xspace}
\newcommand{\DpII}{\mbox{$\mathop{D^{(2)}_p}\limits$}\xspace}
\newcommand{\DpN}{\mbox{$\mathop{D^{(n)}_p}\limits$}\xspace}
\newcommand{\Gp}{\mbox{$\mathop{\mathcal{G}_p}\limits$}\xspace}
\newcommand{\Dq}{\mbox{$\mathop{D_q}\limits$}\xspace}
\newcommand{\DqII}{\mbox{$\mathop{D^{(2)}_q}\limits$}\xspace}
\newcommand{\DqN}{\mbox{$\mathop{D^{(n)}_q}\limits$}\xspace}
\newcommand{\Gq}{\mbox{$\mathop{\mathcal{G}_q}\limits$}\xspace}

% OR
\newcommand{\OR}{\mbox{$\mathop{\mathtt{OR}}\limits$}\xspace}
\newcommand{\ORs}{\mbox{$\mathop{\mathtt{OR}}\limits$s}\xspace}

%Noun
\newcommand{\Myo}{\mbox{$\mathop{\mathtt{Myopathy}}\limits$}\xspace}
\newcommand{\NonMyo}{\mbox{$\mathop{\mathtt{without \ Myopathy}}\limits$}\xspace}

%abbreviation
\newcommand{\cmi}{\mbox{$\mathop{\boldsymbol{c}_i}\limits$}\xspace}
\newcommand{\cmj}{\mbox{$\mathop{\boldsymbol{c}_j}\limits$}\xspace}
\newcommand{\cmADRi}{\mbox{$\mathop{\boldsymbol{c}^{+}_i}\limits$}\xspace}
\newcommand{\cmNoADRi}{\mbox{$\mathop{\boldsymbol{c}^{-}_i}\limits$}\xspace}
\newcommand{\adrs}{\mbox{$\mathop{\text{ADRs}}\limits$}\xspace}
\newcommand{\adr}{\mbox{$\mathop{\text{ADR}}\limits$}\xspace}
\newcommand{\ehrs}{\mbox{$\mathop{\text{EHRs}}\limits$}\xspace}
\newcommand{\ddis}{\mbox{$\mathop{\text{DDIs}}\limits$}\xspace}
\newcommand{\ddi}{\mbox{$\mathop{\text{DDI}}\limits$}\xspace}

%single drug similarity
\newcommand{\SDSd}{\mbox{$\mathop{\text{SDS}_{\text{2d}}}\limits$}\xspace}
\newcommand{\SDSc}{\mbox{$\mathop{\text{SDS}_{\text{cm}}}\limits$}\xspace}
\newcommand{\SDS}{\mbox{$\mathop{\text{SDS}}\limits$}\xspace}
\newcommand{\SDSs}{\mbox{$\mathop{\text{SDSs}}\limits$}\xspace}

%different kernel
%\newcommand{\GMgd}{\mbox{$\mathop{\mathcal{K}_\text{GMgd}}\limits$}\xspace}
\newcommand{\Sgm}{\mbox{$\mathop{\mathcal{S}_\text{gm}}\limits$}\xspace}
\newcommand{\GMop}{\mbox{$\mathop{\mathcal{K}_\text{gm}}\limits$}\xspace}
\newcommand{\GMopcm}{\mbox{$\mathop{\mathcal{K}_\text{gm}^\text{cm}}\limits$}\xspace}
\newcommand{\GMavg}{\mbox{$\mathop{\mathcal{K}_\text{ds}}\limits$}\xspace}
\newcommand{\GMprob}{\mbox{$\mathop{\mathcal{K}_\text{pb}}\limits$}\xspace}
\newcommand{\GMtan}{\mbox{$\mathop{\mathcal{K}_\text{cd}}\limits$}\xspace}
\newcommand{\GMtanorderK}{\mbox{$\mathop{\mathcal{K}^{(k)}_\text{cd}}\limits$}\xspace}
\newcommand{\GMtanorderI}{\mbox{$\mathop{\mathcal{K}^{(1)}_\text{cd}}\limits$}\xspace}
\newcommand{\GMtanorderII}{\mbox{$\mathop{\mathcal{K}^{(2)}_\text{cd}}\limits$}\xspace}

%experiments
\newcommand{\Dall}{\mbox{$\mathop{\mathcal{D}_{\text{FAERS}}}\limits$}\xspace} % toal unique combination in Myopathy and Nonmyopathy (without combination that contain only one drug)
\newcommand{\Dk}{\mbox{$\mathop{\mathcal{D}^{\text{k}}}\limits$}\xspace}
\newcommand{\Dtwok}{\mbox{$\mathop{\mathcal{D}^{\text{2000}}}\limits$}\xspace}
\newcommand{\Dfourk}{\mbox{$\mathop{\mathcal{D}^{\text{4000}}}\limits$}\xspace}
\newcommand{\Dataset}{\mbox{$\mathop{\mathcal{D}^{*}}\limits$}\xspace}
\newcommand{\Dscider}{\mbox{$\mathop{\mathcal{D}_{\text{Myo}}}\limits$}\xspace}

%table
\newcommand{\IID}{\mbox{$\mathop{\text{2d}}\limits$}\xspace}
\newcommand{\coSim}{\mbox{$\mathop{\text{cm}}\limits$}\xspace}
\newcommand{\orderI}{\mbox{$\mathop{\text{ord-}1}\limits$}\xspace}
\newcommand{\orderII}{\mbox{$\mathop{\text{ord-}2}\limits$}\xspace}

%Data set
\newcommand{\Nneg}{\mbox{$\mathop{\mathcal{N}}\limits$}\xspace}  % NonMyopathy unique cases
\newcommand{\Nminus}{\mbox{$\mathop{\mathcal{N}^-}\limits$}\xspace}  % NonMyopathy unique casse
\newcommand{\Nzero}{\mbox{$\mathop{\mathcal{N}^0}\limits$}\xspace}  % NonMyopathy overlaping cases
\newcommand{\Mpos}{\mbox{$\mathop{\mathcal{M}}\limits$}\xspace}  % Myopathy    overlaping cases
\newcommand{\Mzero}{\mbox{$\mathop{\mathcal{M}^0}\limits$}\xspace}  % Myopathy    overlaping cases
\newcommand{\Mplus}{\mbox{$\mathop{\mathcal{M}^+}\limits$}\xspace}  % Myopathy    unique cases
\newcommand{\Nmis}{\mbox{$\mathop{\tilde{\mathcal{N}}^{+}}\limits$}\xspace}
\newcommand{\Mmis}{\mbox{$\mathop{\tilde{\mathcal{M}}^{-}}\limits$}\xspace}  
\newcommand{\Nmist}{\mbox{$\mathop{\tilde{\mathcal{N}}^{10+}}\limits$}\xspace}
\newcommand{\Mmist}{\mbox{$\mathop{\tilde{\mathcal{M}}^{10-}}\limits$}\xspace}   
\newcommand{\Nt}{\mbox{$\mathop{\tilde{\mathcal{N}}^{10-}}\limits$}\xspace}
\newcommand{\Mt}{\mbox{$\mathop{\tilde{\mathcal{M}}^{10+}}\limits$}\xspace} 
\newcommand{\Asix}{\Nminus}  % NonMyopathy unique cases 6k
\newcommand{\Bsix}{\Nzero}  % NonMyopathy overlaping cases 6k
\newcommand{\Csix}{\Mzero}  % Myopathy    overlaping cases 6k
\newcommand{\Dsix}{\Mplus}  % Myopathy    overlaping cases 6k

%\newcommand{\etal}{\mbox{\emph{et al.}}\xspace}
\newcommand{\mytitle}{Drug-drug interaction prediction based on \\co-medication patterns and graph matching}


==> figure/K_cosim_D2k/Freq_A_D/K_cosim_D2k_Freq_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(748,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(748,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(748,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(748,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(748,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(748,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(748,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}1}}%
      \put(1922,484){\makebox(0,0){\strut{}10}}%
      \put(3031,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}frequency}}%
      \csname LTb\endcsname%
      \put(2039,3557){\makebox(0,0)[l]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(2039,3345){\makebox(0,0)[l]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D2k_Freq_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D2k/OR_B_C/K_cosim_D2k_OR_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio}}%
      \csname LTb\endcsname%
      \put(1979,3573){\makebox(0,0)[l]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(1979,3377){\makebox(0,0)[l]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D2k_OR_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D2k/Order_A_D/K_cosim_D2k_Order_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \csname LTb\endcsname%
      \put(2039,3573){\makebox(0,0)[l]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(2039,3377){\makebox(0,0)[l]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D2k_Order_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D2k/Order_B_C/K_cosim_D2k_Order_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \csname LTb\endcsname%
      \put(1979,3573){\makebox(0,0)[l]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(1979,3377){\makebox(0,0)[l]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D2k_Order_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D2k/back_ups/Freq_OR/K_cosim_D2k_freq_or_ABCD.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1015){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1325){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,1636){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,1946){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,2257){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,2567){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1635){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio / frequency}}%
      \put(2443,3557){\makebox(0,0){\strut{}KGMopcoSim combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3155){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2998){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
      \csname LTb\endcsname%
      \put(3536,2841){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2684){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D2k_freq_or_ABCD}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D2k/back_ups/Order/K_cosim_D2k_Order_prediction_value.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \csname LTb\endcsname%
      \put(3716,3573){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3716,3377){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3716,3181){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
      \csname LTb\endcsname%
      \put(3716,2985){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D2k_Order_prediction_value}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D4k/Freq_A_D/K_cosim_D4k_Freq_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(748,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(748,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(748,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(748,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(748,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(748,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(748,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}1}}%
      \put(1922,484){\makebox(0,0){\strut{}10}}%
      \put(3031,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}frequency}}%
      \csname LTb\endcsname%
      \put(2372,3573){\makebox(0,0)[l]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(2372,3377){\makebox(0,0)[l]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D4k_Freq_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D4k/OR_B_C/K_cosim_D4k_OR_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1121){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1538){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,1955){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,2372){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,2789){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,3206){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio}}%
      \csname LTb\endcsname%
      \put(1979,3631){\makebox(0,0)[l]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(1979,3435){\makebox(0,0)[l]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D4k_OR_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D4k/Order_A_D/K_cosim_D4k_Order_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \csname LTb\endcsname%
      \put(2039,3573){\makebox(0,0)[l]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(2039,3377){\makebox(0,0)[l]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D4k_Order_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D4k/Order_B_C/K_cosim_D4k_Order_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \csname LTb\endcsname%
      \put(1979,3573){\makebox(0,0)[l]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(1979,3377){\makebox(0,0)[l]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D4k_Order_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D4k/back_ups/Freq_OR/K_cosim_D4k_freq_or_ABCD.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1015){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1325){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,1636){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,1946){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,2257){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,2567){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1635){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio / frequency}}%
      \put(2443,3557){\makebox(0,0){\strut{}KGMopcoSim combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3155){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2998){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
      \csname LTb\endcsname%
      \put(3536,2841){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2684){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D4k_freq_or_ABCD}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D4k/back_ups/Order/K_cosim_D4k_Order_prediction_value.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1191){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1677){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,2164){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2650){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,3137){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3623){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \csname LTb\endcsname%
      \put(3716,3573){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3716,3377){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3716,3181){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
      \csname LTb\endcsname%
      \put(3716,2985){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{K_cosim_D4k_Order_prediction_value}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/K_cosim_D6k/Order_A_D/temp_linear_x <==
reset


#set term x11
#set term epslatex color size 3.0, 1.5
set term epslatex color size 4.5, 2.25
set output "K_cosim_D6k_Order_vs_Prediction_value_A_D.tex"


set xlabel offset 0, 0
set ylabel offset 0, 0
##set xzeroaxis
##set yzeroaxis

set xtics axis
set ytics axis


set xlabel 'drug order'
set ylabel 'prediction value'



set arrow from 0 , -2.2 to 0 , 4.5   nohead filled size 3, 15
#set arrow from 0 ,  5.0 to 0 ,-3.0   filled size 0.25, 55
set arrow from -0.5 , 0.0 to 85.0 , 0  nohead filled size 3, 15
set arrow from -0.5 , -2.0 to 85.0 , -2.0  nohead filled size 3, 15
#set arrow from 0,0 to -1.1,0   filled size 0.05,15

set size 0.7, 1.2
set xtics nomirror
set ytics nomirror


set nokey

set border 0


##set lmargin at screen 0.1;
##set rmargin at screen 0.95;
##set bmargin at screen 0.1;
##set tmargin at screen 0.95;


##set xtics font "Helvetica,50" 
##set ytics font "Helvetica,10" 
##set x2tics font "Helvetica,10" 
##set y2tics font "Helvetica,10" 
    	
      					
set xrange [0.0:85.0]			
set yrange [-2.0:4.0] 			


#set ytics ('100' 100, '200' 200, '300' 300, '400' 400, '500' 500, '600' 600)
#set xtics offset 0,5
#set xtics ('\scriptsize{-1.0}' -1.0, '\scriptsize{-0.5}' -0.5, '\scriptsize{0}' 0, '\scriptsize{0.5}' 0.5, '\tiny{1.0}' 1.0,)
#set xtics 0,2,14.0

set xtics border
set xtics offset 0,0
set xtics ('0' 0, '10' 10, '20' 20, '30' 30, '40' 40, '50' 50,'60' 60,'70' 70, '80' 80)

#set ytics offset 0.5,0
#set ytics ('\scriptsize{-1.0}' -1.0, '\scriptsize{-0.5}' -0.5, '\scriptsize{0}' 0, '\scriptsize{0.5}' 0.5, '\tiny{1.0}' 1.0,)
set ytics -2,1,4.0

#set arrow from -1,-1 to 1,1 nohead lc rgb 'red' front
#set label 'y=x' at -0.9, -1.0

#set title "KGMopcoSim Unique combination in ${D^{4000}}$" offset 0,1

#set key box opaque height 0.3 width 0.1
set key spacing 2.5
set key samplen 4
set key font ",10"
set key width  15
set key height  1
set key at graph 1.0, 1.05 box 
set key Left reverse
plot 'K_cosim_D6k_Order_vs_Prediction_value_A.txt' w points pt 1 ps 0.5 lc rgb 'blue' title '\Asix non-myopathy' , \
'K_cosim_D6k_Order_vs_Prediction_value_D.txt' w points pt 7 ps 0.5 lc rgb 'goldenrod' title '\Dsix myopathy' 


reset
set term x11
system 'ps2pdf -dEPSCrop K_cosim_D6k_Order_vs_Prediction_value_A_D.eps K_cosim_D6k_Order_vs_Prediction_value_A_D.pdf'


==> figure/back_ups/RBF_1st_D2k/Freq_A_D/RBF_1st_D2k_Freq_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(748,704){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(748,903){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(748,1103){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(748,1302){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(748,1501){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(748,1701){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(748,1900){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(748,2100){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,2299){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(748,2498){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(748,2698){\makebox(0,0)[r]{\strut{}$7$}}%
      \put(748,2897){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(814,484){\makebox(0,0){\strut{}1}}%
      \put(1922,484){\makebox(0,0){\strut{}10}}%
      \put(3031,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1800){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}frequency}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 1st Unique combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3179){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,3022){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D2k_Freq_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_1st_D2k/OR_B_C/RBF_1st_D2k_OR_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(668,903){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1103){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1302){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,1501){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,1701){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,1900){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,2100){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(668,2299){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(668,2498){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(668,2698){\makebox(0,0)[r]{\strut{}$7$}}%
      \put(668,2897){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1800){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio}}%
      \put(2443,3557){\makebox(0,0){\strut{}RBF 1st overlap combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3179){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,3022){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D2k_OR_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_1st_D2k/Order_A_D/RBF_1st_D2k_Order_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(682,996){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1288){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1580){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1872){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2164){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2455){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,2747){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(682,3039){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(682,3331){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(682,3623){\makebox(0,0)[r]{\strut{}$7$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2163){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \csname LTb\endcsname%
      \put(3716,3612){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3716,3455){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D2k_Order_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_1st_D2k/Order_B_C/RBF_1st_D2k_Order_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(682,909){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1115){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1320){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1525){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,1731){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,1936){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,2142){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(682,2347){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(682,2552){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(682,2758){\makebox(0,0)[r]{\strut{}$7$}}%
      \put(682,2963){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1833){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 1st Overlap combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3258){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,3101){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D2k_Order_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_1st_D4k/Freq_A_D_all/RBF_1st_D4k_Freq_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(748,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(748,1073){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(748,1442){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(748,1812){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(748,2181){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(748,2550){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(748,2919){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}1}}%
      \put(1922,484){\makebox(0,0){\strut{}10}}%
      \put(3031,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1811){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}frequency}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 1st Unique combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3205){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,3048){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D4k_Freq_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_1st_D4k/OR_B_C_all/RBF_1st_D4k_OR_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1040){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1376){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,1713){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,2049){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,2385){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,2721){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1712){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio}}%
      \put(2443,3557){\makebox(0,0){\strut{}RBF 1st overlap combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3169){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,3012){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D4k_OR_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_1st_D4k/Order_A_D_all/RBF_1st_D4k_Order_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 1st Unique combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D4k_Order_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_1st_D4k/Order_B_C_all/RBF_1st_D4k_Order_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 1st Overlap combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_1st_D4k_Order_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D2k/Freq_A_D/RBF_2nd_D2k_Freq_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(748,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(748,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(748,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(748,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(748,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(748,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(748,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}1}}%
      \put(1922,484){\makebox(0,0){\strut{}10}}%
      \put(3031,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}frequency}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 2nd Unique combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D2k_Freq_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D2k/OR_B_C/RBF_2nd_D2k_OR_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio}}%
      \put(2443,3557){\makebox(0,0){\strut{}RBF 2nd overlap combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D2k_OR_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D2k/Order_A_D/RBF_2nd_D2k_Order_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 2nd Unique combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D2k_Order_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D2k/Order_B_C/RBF_2nd_D2k_Order_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 2nd Overlap combination in ${D^{2000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D2k_Order_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D4k/Freq_A_D_all/RBF_2nd_D4k_Freq_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(748,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(748,1073){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(748,1442){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(748,1812){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(748,2181){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(748,2550){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(748,2919){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}1}}%
      \put(1922,484){\makebox(0,0){\strut{}10}}%
      \put(3031,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1811){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}frequency}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 2nd Unique combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3205){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,3048){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D4k_Freq_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D4k/OR_B_C_all/RBF_2nd_D4k_OR_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(668,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(668,1040){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(668,1376){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(668,1713){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(668,2049){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(668,2385){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(668,2721){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(748,484){\makebox(0,0){\strut{}0.1}}%
      \put(1596,484){\makebox(0,0){\strut{}1}}%
      \put(2444,484){\makebox(0,0){\strut{}10}}%
      \put(3291,484){\makebox(0,0){\strut{}100}}%
      \put(4139,484){\makebox(0,0){\strut{}1000}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1712){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2443,154){\makebox(0,0){\strut{}odds ratio}}%
      \put(2443,3557){\makebox(0,0){\strut{}RBF 2nd overlap combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3169){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,3012){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D4k_OR_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D4k/Order_A_D_all/RBF_2nd_D4k_Order_vs_Prediction_value_A_D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 2nd Unique combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}A unique NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}D unique Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D4k_Order_vs_Prediction_value_A_D}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/RBF_2nd_D4k/Order_B_C_all/RBF_2nd_D4k_Order_vs_Prediction_value_B_C.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4536.00,3888.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,1088){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,1472){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,1856){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,2239){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2623){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3007){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(814,484){\makebox(0,0){\strut{}0}}%
      \put(1205,484){\makebox(0,0){\strut{}10}}%
      \put(1596,484){\makebox(0,0){\strut{}20}}%
      \put(1988,484){\makebox(0,0){\strut{}30}}%
      \put(2379,484){\makebox(0,0){\strut{}40}}%
      \put(2770,484){\makebox(0,0){\strut{}50}}%
      \put(3161,484){\makebox(0,0){\strut{}60}}%
      \put(3552,484){\makebox(0,0){\strut{}70}}%
      \put(3943,484){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1855){\rotatebox{-270}{\makebox(0,0){\strut{}prediction value}}}%
      \put(2476,154){\makebox(0,0){\strut{}drug orders}}%
      \put(2476,3557){\makebox(0,0){\strut{}RBF 2nd Overlap combination in ${D^{4000}}$}}%
      \csname LTb\endcsname%
      \put(3536,3080){\makebox(0,0)[r]{\strut{}B overlap NonMyopathy}}%
      \csname LTb\endcsname%
      \put(3536,2923){\makebox(0,0)[r]{\strut{}C overlap Myopathy}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{RBF_2nd_D4k_Order_vs_Prediction_value_B_C}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figure/back_ups/template/ranking_diff.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6480.00,3240.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3350,704){\makebox(0,0)[r]{\strut{}\scriptsize{-1.0}}}%
      \put(3350,1272){\makebox(0,0)[r]{\strut{}\scriptsize{-0.5}}}%
      \put(3350,1840){\makebox(0,0)[r]{\strut{}\scriptsize{0}}}%
      \put(3350,2407){\makebox(0,0)[r]{\strut{}\scriptsize{0.5}}}%
      \put(3350,2975){\makebox(0,0)[r]{\strut{}\tiny{1.0}}}%
      \put(748,1667){\makebox(0,0){\strut{}\scriptsize{-1.0}}}%
      \put(2082,1667){\makebox(0,0){\strut{}\scriptsize{-0.5}}}%
      \put(3416,1667){\makebox(0,0){\strut{}\scriptsize{0}}}%
      \put(4749,1667){\makebox(0,0){\strut{}\scriptsize{0.5}}}%
      \put(6083,1667){\makebox(0,0){\strut{}\tiny{1.0}}}%
      \csname LTb\endcsname%
      \put(1015,704){\makebox(0,0)[l]{\strut{}y=x}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1839){\rotatebox{-270}{\makebox(0,0){\strut{}$Q$ ranking difference}}}%
      \put(3415,154){\makebox(0,0){\strut{}$Q$ ranking difference}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ranking_diff}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results_table/ABCD_average_6k_info.tex <==
\begin{table}[!h]
  \caption{Statistical Information in \DVIk }
  \label{table:Statis_D_6k}
  \centering
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{2pt}}l@{\hspace{10pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}          
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	}
        \hline\hline
				& \Asix	& \Bsix   	& \Csix  & \Dsix	\\
        \hline

	average order		& 2.6777 & 2.3505 & 3.8088 & 7.6150	\\
	average freqency	& 42.0818  & 225.3172      & 20.5653    & 5.5200	\\
	average OR 		& -      & 0.5460 &  31.9983 & -	\\


        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  There are 2,200, 1,264, 2,464 and 1,000 different drug combinations in 
	  \AALL,\BALL,\CALL and \DALL, respectively.
          %\par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}
%


==> results_table/back_ups/ABCD_average_info.tex <==
\begin{table}[!h]
  \caption{Statistical Data Analysis in \DIVk }
  \label{table:Statis_D_4k}
  \centering
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{2pt}}l@{\hspace{10pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}          
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	}
        \hline\hline
				& \A	& \B   	& \C  & \D 	\\
        \hline

	average order		& 2.5850       	 		& 2.3400        & 3.8830        & 7.6150	\\
	average freqency	& 62.5450       		& 264.8980      & 33.9160       & 5.5200	\\
	average OR 		& -			        & 0.4513        & 47.0378       & -		\\


        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  Average frequency in \B and \C are average of sum of duplicated events in \Myo (case) and \NonMyo (control) events.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}
%


==> results_table/back_ups/AD_average_info.tex <==
\begin{table}[!h]
  \caption{statistical data analysis in \DIIk }
  \label{table:Statis_D_2k}
  \centering
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{2pt}}l@{\hspace{10pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}          
	@{\hspace{2pt}}r@{\hspace{2pt}}
	}
        \hline\hline
				& \A	   	  & \D 	\\
        \hline

	average order		& 2.5850     & 7.6150       \\
	average freqency	& 62.5450     & 5.5200       \\
	%average OR 		& -     & -		\\


        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		The average order is the mean of the drug's number in all combinations in \A and \D, respectively.
		The average frequency is the mean of the frequencies (number of duplicated events) in all combination in \A and \D.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}
%


==> results_table/back_ups/Enrichment.tex <==
\begin{table}[!h]
  \centering
  \caption{ mean percentage of missclassification percentage }
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
%	{p{25mm}|p{10mm}|p{10mm}|p{10mm}
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}   
	@{\hspace{8pt}}r@{\hspace{8pt}}       
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{D}^{{2000}}$ & $\mathcal{D}^{{4000}}$	& $\mathcal{D}^{{6948}}$	\\
        \hline
	Top-10  miss   & 0.1742  & 0.3095   &	0.3071 \\	
	Top-all miss   & 0.1671  & 0.1830   &   0.1856	\\	
	All negative   & 0.1412  & 0.1513   &   0.1557	\\	
	All positive   & 0.2080	 & 0.2510   &	0.2425 \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  percentage is calculated by the number of single drugs which can cause Myopathy itself / drug number of combinations
	  Top-10  miss is the top-10 prediction value which is negative label
	  Top-all miss is the all positive predtion value which is nagative label
	  All negative is all negative label
          All positive is all positive label
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}
%


==> results_table/back_ups/drug_freq_D2k.tex <==
\begin{table*}[!h]
  \centering
  \caption{ single drug frequency of  $\mathcal{D}^{{2000}}$ }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
 values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\
        \hline
3837 &0.2087 &acetylsalicylicacid      &232 &0.2320 &\textbf{simvastatin}      &3200 &0.1520 &prednisolone     &46 &0.0460 &acetaminophen \\
3609 &0.1963 &acetaminophen    &228 &0.2280 &acetylsalicylicacid       &1961 &0.0931 &\textbf{phenytoin}       &45 &0.0450 &metformin \\
3330 &0.1811 &\textbf{simvastatin}     &179 &0.1790 &acetaminophen     &1921 &0.0912 &capecitabine     &44 &0.0440 &warfarin \\
2849 &0.1550 &levothyroxine    &161 &0.1610 &\textbf{atorvastatin}     &1312 &0.0623 &melphalan        &43 &0.0430 &acetylsalicylicacid \\
2709 &0.1474 &gabapentin       &122 &0.1220 &furosemide        &1253 &0.0595 &alendronate      &38 &0.0380 &cyclophosphamide \\
2639 &0.1436 &alprazolam       &110 &0.1100 &amlodipine        &1243 &0.0590 &diazepam         &36 &0.0360 &\textbf{dexamethasone} \\
2522 &0.1372 &\textbf{atorvastatin}    &108 &0.1080 &omeprazole        &1050 &0.0499 &cetirizine       &30 &0.0300 &prednisolone \\
2366 &0.1287 &clonazepam       &86 &0.0860 &levothyroxine      &966 &0.0459 &lamotrigine       &28 &0.0280 &cisplatin \\
2333 &0.1269 &\textbf{dexamethasone}   &83 &0.0830 &atenolol   &879 &0.0418 &valproicacid      &27 &0.0270 &valproicacid \\
2201 &0.1197 &prochlorperazine         &80 &0.0800 &gabapentin         &792 &0.0376 &salbutamol        &27 &0.0270 &prednisone \\
2114 &0.1150 &furosemide       &79 &0.0790 &metoprolol         &744 &0.0353 &acetaminophen     &26 &0.0260 &methotrexate \\
2045 &0.1112 &oxycodone        &73 &0.0730 &hydrocodone        &702 &0.0333 &acetylsalicylicacid       &24 &0.0240 &doxorubicin \\
1832 &0.0997 &valaciclovir     &72 &0.0720 &alprazolam         &694 &0.0330 &cisplatin         &24 &0.0240 &quetiapine \\
1815 &0.0987 &\textbf{fentanyl}        &71 &0.0710 &lansoprazole       &688 &0.0327 &ethinylestradiol  &23 &0.0230 &\textbf{zidovudine} \\
1739 &0.0946 &amitriptyline    &70 &0.0700 &oxycodone  &669 &0.0318 &\textbf{olanzapine}       &23 &0.0230 &ibuprofen \\
1709 &0.0930 &atenolol         &70 &0.0700 &alendronate        &667 &0.0317 &cyclosporine      &22 &0.0220 &cetuximab \\
1694 &0.0922 &\textbf{pregabalin}      &69 &0.0690 &lisinopril         &652 &0.0310 &warfarin  &22 &0.0220 &\textbf{ritonavir} \\
1660 &0.0903 &omeprazole       &68 &0.0680 &clopidogrel        &632 &0.0300 &tiotropium        &21 &0.0210 &salbutamol \\
1579 &0.0859 &hydrochlorothiazide      &65 &0.0650 &ramipril   &559 &0.0266 &\textbf{fentanyl}         &21 &0.0210 &exenatide \\
1573 &0.0856 &amlodipine       &63 &0.0630 &metformin  &556 &0.0264 &fluticasonepropionate     &20 &0.0200 &cyclosporine \\

total & 18383 &&total & 27387 &&total & 1475840 &&total & 621449 & \\
	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/drug_freq_D4k.tex <==
\begin{table*}[!h]
  \centering
  \caption{ single drug frequency of  $\mathcal{D}^{{4000}}$  }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
 values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\
        \hline
8285 &0.2101 &\textbf{atorvastatin}    &399 &0.1995 &\textbf{simvastatin}      &27550 &0.0841 &ethinylestradiol        &92 &0.0460 &acetylsalicylicacid \\
7430 &0.1884 &\textbf{simvastatin}     &350 &0.1750 &acetylsalicylicacid       &23265 &0.0711 &metformin       &90 &0.0450 &metformin \\
5239 &0.1328 &alendronate      &332 &0.1660 &\textbf{atorvastatin}     &18275 &0.0558 &conjugatedestrogens     &81 &0.0405 &acetaminophen \\
3759 &0.0953 &acetylsalicylicacid      &258 &0.1290 &acetaminophen     &17433 &0.0532 &medroxyprogesterone     &76 &0.0380 &warfarin \\
3698 &0.0938 &\textbf{ezetimibe}       &162 &0.0810 &amlodipine        &15933 &0.0487 &exenatide       &59 &0.0295 &cyclophosphamide \\
3577 &0.0907 &\textbf{rosuvastatin}    &162 &0.0810 &alendronate       &14170 &0.0433 &norelgestromin  &59 &0.0295 &exenatide \\
2470 &0.0626 &levothyroxine    &158 &0.0790 &levothyroxine     &13633 &0.0416 &acetaminophen   &57 &0.0285 &\textbf{dexamethasone} \\
2364 &0.0599 &amlodipine       &152 &0.0760 &omeprazole        &13158 &0.0402 &fluticasonepropionate   &56 &0.0280 &quetiapine \\
2240 &0.0568 &misoprostol      &149 &0.0745 &furosemide        &12764 &0.0390 &salmeterol      &54 &0.0270 &prednisone \\
2023 &0.0513 &teriparatide     &126 &0.0630 &metoprolol        &11880 &0.0363 &acetylsalicylicacid     &51 &0.0255 &prednisolone \\
1928 &0.0489 &acetaminophen    &126 &0.0630 &\textbf{rosuvastatin}     &9230 &0.0282 &rosiglitazone    &50 &0.0250 &valproicacid \\
1534 &0.0389 &trimethoprim     &125 &0.0625 &atenolol  &8722 &0.0266 &cisplatin        &48 &0.0240 &varenicline \\
1531 &0.0388 &mifepristone     &109 &0.0545 &\textbf{ezetimibe}        &8287 &0.0253 &warfarin         &47 &0.0235 &cisplatin \\
1400 &0.0355 &sulfamethoxazole         &108 &0.0540 &lisinopril        &8209 &0.0251 &budesonide       &45 &0.0225 &\textbf{paroxetine} \\
1335 &0.0339 &ibandronate      &105 &0.0525 &hydrocodone       &8088 &0.0247 &drospirenone     &43 &0.0215 &lamotrigine \\
1324 &0.0336 &calcium  &103 &0.0515 &gabapentin        &7903 &0.0241 &insulinglargine  &42 &0.0210 &insulinglargine \\
1299 &0.0329 &\textbf{niacin}  &102 &0.0510 &clopidogrel       &7647 &0.0234 &\textbf{dexamethasone}   &42 &0.0210 &cyclosporine \\
1290 &0.0327 &prednisone       &101 &0.0505 &metformin         &7578 &0.0231 &quetiapine       &42 &0.0210 &\textbf{ritonavir} \\
1194 &0.0303 &omeprazole       &96 &0.0480 &alprazolam         &7490 &0.0229 &salbutamol       &41 &0.0205 &doxorubicin \\
1169 &0.0296 &doxycycline      &94 &0.0470 &oxycodone  &7402 &0.0226 &formoterol       &41 &0.0205 &ibuprofen \\


	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/drug_freq_D6k.tex <==
\begin{table*}[!h]
  \centering
  \caption{ single drug frequency of  $\mathcal{D}^{{6000}}$  }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
 values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\
        \hline
10439 &0.1858 &\textbf{atorvastatin}   &535 &0.1544 &acetylsalicylicacid       &28064 &0.0744 &ethinylestradiol        &179 &0.0517 &acetylsalicylicacid \\
9050 &0.1611 &\textbf{simvastatin}     &532 &0.1536 &\textbf{atorvastatin}     &24765 &0.0656 &metformin       &170 &0.0491 &acetaminophen \\
6015 &0.1070 &alendronate      &522 &0.1507 &\textbf{simvastatin}      &18575 &0.0492 &conjugatedestrogens     &148 &0.0427 &metformin \\
5755 &0.1024 &acetylsalicylicacid      &362 &0.1045 &acetaminophen     &17506 &0.0464 &medroxyprogesterone     &124 &0.0358 &warfarin \\
5131 &0.0913 &\textbf{rosuvastatin}    &265 &0.0765 &levothyroxine     &16981 &0.0450 &acetaminophen   &102 &0.0294 &quetiapine \\
4057 &0.0722 &\textbf{ezetimibe}       &259 &0.0748 &amlodipine        &16424 &0.0435 &exenatide       &102 &0.0294 &\textbf{dexamethasone} \\
3711 &0.0660 &levothyroxine    &228 &0.0658 &\textbf{rosuvastatin}     &15212 &0.0403 &acetylsalicylicacid     &95 &0.0274 &valproicacid \\
3165 &0.0563 &teriparatide     &223 &0.0644 &alendronate       &14470 &0.0383 &norelgestromin  &91 &0.0263 &cyclophosphamide \\
2967 &0.0528 &amlodipine       &217 &0.0626 &omeprazole        &14126 &0.0374 &fluticasonepropionate   &86 &0.0248 &prednisone \\
2719 &0.0484 &acetaminophen    &205 &0.0592 &furosemide        &13566 &0.0359 &salmeterol      &86 &0.0248 &ibuprofen \\
2257 &0.0402 &misoprostol      &195 &0.0563 &metoprolol        &9691 &0.0257 &rosiglitazone    &80 &0.0231 &levothyroxine \\
2070 &0.0368 &metoprolol       &174 &0.0502 &metformin         &9587 &0.0254 &warfarin         &80 &0.0231 &lamotrigine \\
1908 &0.0340 &\textbf{niacin}  &174 &0.0502 &atenolol  &9234 &0.0245 &cisplatin        &79 &0.0228 &\textbf{ritonavir} \\
1745 &0.0311 &omeprazole       &170 &0.0491 &lisinopril        &9144 &0.0242 &quetiapine       &78 &0.0225 &exenatide \\
1659 &0.0295 &trimethoprim     &159 &0.0459 &\textbf{ezetimibe}        &8774 &0.0232 &\textbf{dexamethasone}   &76 &0.0219 &varenicline \\
1606 &0.0286 &lisinopril       &155 &0.0447 &hydrochlorothiazide       &8528 &0.0226 &budesonide       &74 &0.0214 &\textbf{lamivudine} \\
1570 &0.0279 &ibandronate      &154 &0.0445 &hydrocodone       &8469 &0.0224 &drospirenone     &74 &0.0214 &prednisolone \\
1557 &0.0277 &prednisone       &152 &0.0439 &clopidogrel       &8351 &0.0221 &insulinglargine  &70 &0.0202 &cyclosporine \\
1557 &0.0277 &clopidogrel      &142 &0.0410 &gabapentin        &8210 &0.0218 &salbutamol       &70 &0.0202 &\textbf{paroxetine} \\
1531 &0.0272 &mifepristone     &139 &0.0401 &alprazolam        &8088 &0.0214 &\textbf{ritonavir}       &68 &0.0196 &salbutamol \\
	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/drug_freq_all.tex <==
\begin{table*}[!h]
  \centering
  \caption{ single drug frequency of  all  }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}l@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}   
	@{\hspace{2pt}}l@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}l@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
	values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\% &M freq pair & M uniq pair &N freq pair & N uniq pair		\\
        \hline
11068 &0.1706 &acetylsalicylicacid     &6190 &0.2260 &acetylsalicylicacid      &168214 &0.1140 &acetylsalicylicacid    &101556 &0.1634 &acetylsalicylicacid \\
9671 &0.1490 &\textbf{simvastatin}     &4224 &0.1542 &\textbf{atorvastatin}    &130558 &0.0885 &acetaminophen  &73208 &0.1178 &acetaminophen \\
9221 &0.1421 &\textbf{atorvastatin}    &4127 &0.1507 &\textbf{simvastatin}     &99394 &0.0673 &metformin       &66285 &0.1067 &furosemide \\
6967 &0.1074 &acetaminophen    &3949 &0.1442 &acetaminophen    &95735 &0.0649 &furosemide      &57453 &0.0925 &levothyroxine \\
5736 &0.0884 &levothyroxine    &3278 &0.1197 &levothyroxine    &89984 &0.0610 &levothyroxine   &50753 &0.0817 &\textbf{atorvastatin} \\
4868 &0.0750 &furosemide       &3072 &0.1122 &furosemide       &83631 &0.0567 &\textbf{atorvastatin}   &50535 &0.0813 &\textbf{simvastatin} \\
4849 &0.0747 &amlodipine       &2774 &0.1013 &metoprolol       &80422 &0.0545 &amlodipine      &49762 &0.0801 &metformin \\
4584 &0.0706 &\textbf{rosuvastatin}    &2591 &0.0946 &amlodipine       &78731 &0.0533 &\textbf{simvastatin}    &49673 &0.0799 &metoprolol \\
4543 &0.0700 &metoprolol       &2460 &0.0898 &hydrochlorothiazide      &73666 &0.0499 &metoprolol      &47891 &0.0771 &amlodipine \\
4282 &0.0660 &omeprazole       &2451 &0.0895 &omeprazole       &72415 &0.0491 &omeprazole      &46343 &0.0746 &omeprazole \\
4108 &0.0633 &metformin        &2420 &0.0884 &lisinopril       &65124 &0.0441 &warfarin        &43342 &0.0697 &lisinopril \\
4006 &0.0617 &hydrochlorothiazide      &2332 &0.0851 &metformin        &64901 &0.0440 &lisinopril      &39650 &0.0638 &hydrochlorothiazide \\
3950 &0.0609 &lisinopril       &2281 &0.0833 &\textbf{rosuvastatin}    &62686 &0.0425 &hydrochlorothiazide     &37536 &0.0604 &warfarin \\
3697 &0.0570 &\textbf{ezetimibe}       &2100 &0.0767 &clopidogrel      &58859 &0.0399 &salbutamol      &35216 &0.0567 &salbutamol \\
3498 &0.0539 &clopidogrel      &2002 &0.0731 &atenolol         &52130 &0.0353 &clopidogrel     &32303 &0.0520 &clopidogrel \\
3445 &0.0531 &atenolol         &1744 &0.0637 &esomeprazole     &51637 &0.0350 &fluticasonepropionate   &31168 &0.0502 &esomeprazole \\
2857 &0.0440 &esomeprazole     &1715 &0.0626 &salbutamol       &50510 &0.0342 &esomeprazole    &30932 &0.0498 &atenolol \\
2854 &0.0440 &gabapentin       &1709 &0.0624 &hydrocodone      &48510 &0.0329 &prednisone      &28342 &0.0456 &alprazolam \\
2842 &0.0438 &alendronate      &1697 &0.0620 &gabapentin       &48102 &0.0326 &alprazolam      &28076 &0.0452 &gabapentin \\
2841 &0.0438 &hydrocodone      &1684 &0.0615 &\textbf{ezetimibe}       &47256 &0.0320 &atenolol        &26955 &0.0434 &hydrocodone \\
%total & 64892 &&total & 27387 &&total & 1475840 &&total & 621449 & \\

	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/drug_freq_pair_D2k.tex <==
\begin{table*}[!h]
  \centering
  \caption{ pair drug frequency of  $\mathcal{D}^{{2000}}$  }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\
        \hline
2100 &0.1142 &acetaminophen gabapentin         &96 &0.0960 &acetylsalicylicacid \textbf{simvastatin}   &1850 &0.0879 &capecitabine \textbf{phenytoin}  &16 &0.0160 &\textbf{ritonavir} \textbf{zidovudine} \\
1957 &0.1065 &\textbf{dexamethasone} prochlorperazine  &63 &0.0630 &acetaminophen hydrocodone  &1151 &0.0547 &melphalan prednisolone   &14 &0.0140 &lopinavir \textbf{ritonavir} \\
1866 &0.1015 &acetylsalicylicacid \textbf{simvastatin}         &55 &0.0550 &acetylsalicylicacid \textbf{atorvastatin}  &1137 &0.0540 &alendronate prednisolone         &13 &0.0130 &\textbf{lamivudine} \textbf{zidovudine} \\
1847 &0.1005 &acetaminophen clonazepam         &46 &0.0460 &acetylsalicylicacid amlodipine     &661 &0.0314 &diazepam lamotrigine      &13 &0.0130 &acetaminophen hydrocodone \\
1755 &0.0955 &acetaminophen valaciclovir       &44 &0.0440 &acetaminophen oxycodone    &486 &0.0231 &ethinylestradiol norelgestromin   &12 &0.0120 &\textbf{emtricitabine} \textbf{tenofovir} \\
1711 &0.0931 &clonazepam gabapentin    &42 &0.0420 &omeprazole \textbf{simvastatin}    &456 &0.0217 &\textbf{nifedipine} olmesartan    &11 &0.0110 &insulinglargine metformin \\
1657 &0.0901 &gabapentin valaciclovir  &41 &0.0410 &acetaminophen acetylsalicylicacid  &433 &0.0206 &cyclosporine prednisolone         &11 &0.0110 &lopinavir \textbf{zidovudine} \\
1614 &0.0878 &clonazepam valaciclovir  &39 &0.0390 &acetylsalicylicacid furosemide     &427 &0.0203 &fluticasonepropionate salmeterol  &10 &0.0100 &\textbf{ritonavir} \textbf{tenofovir} \\
1609 &0.0875 &\textbf{fentanyl} gabapentin     &37 &0.0370 &acetaminophen zoledronate  &422 &0.0200 &cetuximab cisplatin       &10 &0.0100 &cyclophosphamide vincristine \\
1586 &0.0863 &acetaminophen \textbf{fentanyl}  &37 &0.0370 &furosemide \textbf{simvastatin}    &419 &0.0199 &cetirizine ethinylestradiol       &10 &0.0100 &conjugatedestrogens medroxyprogesterone \\
1494 &0.0813 &acetaminophen \textbf{dexamethasone}     &37 &0.0370 &acetylsalicylicacid ramipril       &419 &0.0199 &cetirizine norelgestromin         &10 &0.0100 &folicacid pemetrexed \\
1478 &0.0804 &amitriptyline gabapentin         &35 &0.0350 &acetaminophen \textbf{simvastatin}         &418 &0.0199 &\textbf{olanzapine} valproicacid  &10 &0.0100 &\textbf{lamivudine} \textbf{ritonavir} \\
1470 &0.0800 &\textbf{dexamethasone} gabapentin        &35 &0.0350 &acetylsalicylicacid metoprolol     &403 &0.0191 &diazepam valproicacid     &10 &0.0100 &cyclophosphamide doxorubicin \\
1438 &0.0782 &clonazepam prochlorperazine      &35 &0.0350 &acetylsalicylicacid clopidogrel    &401 &0.0190 &salbutamol salmeterol     &10 &0.0100 &exenatide metformin \\
1428 &0.0777 &acetaminophen amitriptyline      &34 &0.0340 &ramipril \textbf{simvastatin}      &398 &0.0189 &cisplatin pemetrexed      &9 &0.0090 &cyclophosphamide \textbf{dexamethasone} \\
1387 &0.0755 &alprazolam oxycodone     &34 &0.0340 &amlodipine \textbf{simvastatin}    &398 &0.0189 &diazepam \textbf{olanzapine}      &8 &0.0080 &\textbf{tenofovir} \textbf{zidovudine} \\
1353 &0.0736 &acetaminophen prochlorperazine   &33 &0.0330 &acetaminophen omeprazole   &396 &0.0188 &fluticasonepropionate salbutamol  &8 &0.0080 &cyclophosphamide etoposide \\
1322 &0.0719 &\textbf{dexamethasone} lenalidomide      &32 &0.0320 &acetylsalicylicacid atenolol       &392 &0.0186 &cetirizine salbutamol     &8 &0.0080 &\textbf{emtricitabine} \textbf{ritonavir} \\
1318 &0.0717 &amitriptyline clonazepam         &32 &0.0320 &acetylsalicylicacid omeprazole     &390 &0.0185 &cetirizine fluticasonepropionate  &8 &0.0080 &fluticasonepropionate salmeterol \\
1311 &0.0713 &gabapentin prochlorperazine      &32 &0.0320 &\textbf{atorvastatin} \textbf{simvastatin}         &390 &0.0185 &cetirizine salmeterol     &8 &0.0080 &acetylsalicylicacid clopidogrel \\


	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/drug_freq_pair_D4k.tex <==
\begin{table*}[!h]
  \centering
  \caption{ pair drug frequency of   $\mathcal{D}^{{4000}}$ }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\
        \hline
2383 &0.0604 &\textbf{ezetimibe} \textbf{simvastatin}  &124 &0.0620 &acetylsalicylicacid \textbf{simvastatin}  &17117 &0.0523 &conjugatedestrogens medroxyprogesterone         &29 &0.0145 &exenatide metformin \\
1531 &0.0388 &mifepristone misoprostol         &93 &0.0465 &acetaminophen hydrocodone  &14170 &0.0433 &ethinylestradiol norelgestromin         &22 &0.0110 &\textbf{lamivudine} \textbf{zidovudine} \\
1447 &0.0367 &amlodipine \textbf{atorvastatin}         &90 &0.0450 &acetylsalicylicacid \textbf{atorvastatin}  &12147 &0.0371 &fluticasonepropionate salmeterol        &22 &0.0110 &\textbf{emtricitabine} \textbf{tenofovir} \\
1392 &0.0353 &sulfamethoxazole trimethoprim    &58 &0.0290 &acetylsalicylicacid amlodipine     &10989 &0.0336 &exenatide metformin     &22 &0.0110 &acetaminophen hydrocodone \\
1280 &0.0325 &alendronate ibandronate  &57 &0.0285 &acetaminophen oxycodone    &7573 &0.0231 &metformin rosiglitazone  &21 &0.0105 &lopinavir \textbf{ritonavir} \\
1265 &0.0321 &acetylsalicylicacid \textbf{atorvastatin}        &56 &0.0280 &acetylsalicylicacid metoprolol     &7243 &0.0221 &budesonide formoterol    &20 &0.0100 &\textbf{ritonavir} \textbf{tenofovir} \\
1046 &0.0265 &doxycycline misoprostol  &54 &0.0270 &acetaminophen acetylsalicylicacid  &6836 &0.0209 &drospirenone ethinylestradiol    &20 &0.0100 &fluticasonepropionate salmeterol \\
1045 &0.0265 &acetylsalicylicacid \textbf{simvastatin}         &51 &0.0255 &acetylsalicylicacid clopidogrel    &5064 &0.0155 &ethinylestradiol etonogestrel    &19 &0.0095 &\textbf{ritonavir} \textbf{zidovudine} \\
857 &0.0217 &\textbf{atorvastatin} \textbf{simvastatin}        &50 &0.0250 &omeprazole \textbf{simvastatin}    &4324 &0.0132 &\textbf{lamivudine} \textbf{zidovudine}  &19 &0.0095 &cyclophosphamide doxorubicin \\
775 &0.0197 &alendronate risedronate   &50 &0.0250 &\textbf{atorvastatin} \textbf{simvastatin}         &4171 &0.0127 &buprenorphine naloxone   &16 &0.0080 &insulinglargine metformin \\
636 &0.0161 &\textbf{atorvastatin} \textbf{ezetimibe}  &49 &0.0245 &amlodipine \textbf{simvastatin}    &4073 &0.0124 &\textbf{emtricitabine} \textbf{tenofovir}        &16 &0.0080 &cyclophosphamide vincristine \\
629 &0.0159 &alendronate levothyroxine         &48 &0.0240 &acetylsalicylicacid ramipril       &3908 &0.0119 &acetaminophen hydrocodone        &16 &0.0080 &\textbf{lamivudine} \textbf{ritonavir} \\
608 &0.0154 &alendronate calcium       &48 &0.0240 &amlodipine \textbf{atorvastatin}   &3828 &0.0117 &lopinavir \textbf{ritonavir}     &15 &0.0075 &doxorubicin vincristine \\
568 &0.0144 &\textbf{atorvastatin} \textbf{rosuvastatin}       &46 &0.0230 &acetylsalicylicacid furosemide     &3657 &0.0112 &carboplatin paclitaxel   &15 &0.0075 &exenatide insulinglargine \\
554 &0.0140 &acetylsalicylicacid \textbf{rosuvastatin}         &46 &0.0230 &\textbf{ezetimibe} \textbf{simvastatin}    &3431 &0.0105 &celecoxib \textbf{rofecoxib}     &14 &0.0070 &conjugatedestrogens medroxyprogesterone \\
506 &0.0128 &acetaminophen hydrocodone         &45 &0.0225 &ramipril \textbf{simvastatin}      &3369 &0.0103 &hydrochlorothiazide valsartan    &14 &0.0070 &\textbf{emtricitabine} \textbf{ritonavir} \\
479 &0.0121 &calcium teriparatide      &43 &0.0215 &acetylsalicylicacid atenolol       &3310 &0.0101 &bosentan sildenafil      &13 &0.0065 &metformin rosiglitazone \\
475 &0.0120 &\textbf{atorvastatin} clopidogrel         &42 &0.0210 &acetaminophen omeprazole   &3260 &0.0100 &acetylsalicylicacid \textbf{niacin}      &13 &0.0065 &fluorouracil leucovorin \\
474 &0.0120 &amlodipine \textbf{simvastatin}   &41 &0.0205 &acetaminophen zoledronate  &3209 &0.0098 &fluticasonepropionate salbutamol         &13 &0.0065 &acetylsalicylicacid clopidogrel \\
464 &0.0118 &acetylsalicylicacid clopidogrel   &41 &0.0205 &metoprolol \textbf{simvastatin}    &3153 &0.0096 &insulinglargine insulinlispro    &12 &0.0060 &folicacid pemetrexed \\


	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/drug_freq_pair_D6k.tex <==
\begin{table*}[!h]
  \centering
  \caption{ pair drug frequency of   $\mathcal{D}^{{6000}}$ }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\
        \hline
2560 &0.0456 &\textbf{ezetimibe} \textbf{simvastatin}  &153 &0.0442 &acetylsalicylicacid \textbf{simvastatin}  &17190 &0.0456 &conjugatedestrogens medroxyprogesterone         &42 &0.0121 &\textbf{lamivudine} \textbf{zidovudine} \\
1768 &0.0315 &acetylsalicylicacid \textbf{simvastatin}         &140 &0.0404 &acetylsalicylicacid \textbf{atorvastatin}         &14470 &0.0383 &ethinylestradiol norelgestromin         &40 &0.0115 &exenatide metformin \\
1676 &0.0298 &acetylsalicylicacid \textbf{atorvastatin}        &133 &0.0384 &acetaminophen hydrocodone         &12877 &0.0341 &fluticasonepropionate salmeterol        &37 &0.0107 &\textbf{lamivudine} \textbf{ritonavir} \\
1625 &0.0289 &amlodipine \textbf{atorvastatin}         &83 &0.0240 &acetylsalicylicacid metoprolol     &11248 &0.0298 &exenatide metformin     &36 &0.0104 &\textbf{ritonavir} \textbf{tenofovir} \\
1531 &0.0272 &mifepristone misoprostol         &81 &0.0234 &acetylsalicylicacid amlodipine     &7733 &0.0205 &metformin rosiglitazone  &36 &0.0104 &acetaminophen hydrocodone \\
1474 &0.0262 &sulfamethoxazole trimethoprim    &80 &0.0231 &acetaminophen oxycodone    &7458 &0.0198 &budesonide formoterol    &36 &0.0104 &lopinavir \textbf{ritonavir} \\
1284 &0.0228 &alendronate ibandronate  &73 &0.0211 &amlodipine \textbf{atorvastatin}   &6963 &0.0185 &drospirenone ethinylestradiol    &35 &0.0101 &\textbf{ritonavir} \textbf{zidovudine} \\
1046 &0.0186 &doxycycline misoprostol  &72 &0.0208 &acetylsalicylicacid clopidogrel    &5151 &0.0136 &ethinylestradiol etonogestrel    &35 &0.0101 &\textbf{emtricitabine} \textbf{tenofovir} \\
896 &0.0159 &\textbf{atorvastatin} \textbf{simvastatin}        &69 &0.0199 &acetaminophen acetylsalicylicacid  &5001 &0.0133 &\textbf{lamivudine} \textbf{zidovudine}  &35 &0.0101 &fluticasonepropionate salmeterol \\
849 &0.0151 &alendronate risedronate   &68 &0.0196 &\textbf{ezetimibe} \textbf{simvastatin}    &4797 &0.0127 &acetaminophen hydrocodone        &29 &0.0084 &acetylsalicylicacid clopidogrel \\
792 &0.0141 &alendronate levothyroxine         &65 &0.0188 &acetylsalicylicacid ramipril       &4394 &0.0116 &\textbf{emtricitabine} \textbf{tenofovir}        &25 &0.0072 &cyclophosphamide doxorubicin \\
771 &0.0137 &acetaminophen hydrocodone         &62 &0.0179 &acetylsalicylicacid atenolol       &4295 &0.0114 &lopinavir \textbf{ritonavir}     &25 &0.0072 &\textbf{atazanavir} \textbf{ritonavir} \\
737 &0.0131 &metoprolol \textbf{rosuvastatin}  &59 &0.0170 &\textbf{atorvastatin} \textbf{simvastatin}         &4274 &0.0113 &buprenorphine naloxone   &23 &0.0066 &insulinglargine metformin \\
723 &0.0129 &acetylsalicylicacid \textbf{rosuvastatin}         &58 &0.0167 &omeprazole \textbf{simvastatin}    &3897 &0.0103 &carboplatin paclitaxel   &23 &0.0066 &acetaminophen oxycodone \\
718 &0.0128 &\textbf{niacin} \textbf{simvastatin}      &58 &0.0167 &amlodipine \textbf{simvastatin}    &3457 &0.0092 &celecoxib \textbf{rofecoxib}     &23 &0.0066 &\textbf{emtricitabine} \textbf{ritonavir} \\
713 &0.0127 &acetylsalicylicacid clopidogrel   &57 &0.0165 &acetylsalicylicacid furosemide     &3401 &0.0090 &fluticasonepropionate salbutamol         &23 &0.0066 &ethinylestradiol norelgestromin \\
687 &0.0122 &\textbf{atorvastatin} \textbf{ezetimibe}  &55 &0.0159 &acetaminophen gabapentin   &3383 &0.0090 &acetylsalicylicacid \textbf{niacin}      &22 &0.0064 &lopinavir \textbf{zidovudine} \\
679 &0.0121 &\textbf{atorvastatin} clopidogrel         &54 &0.0156 &\textbf{atorvastatin} metformin    &3369 &0.0089 &hydrochlorothiazide valsartan    &21 &0.0061 &cyclophosphamide vincristine \\
658 &0.0117 &alendronate calcium       &53 &0.0153 &metoprolol \textbf{simvastatin}    &3310 &0.0088 &bosentan sildenafil      &21 &0.0061 &exenatide insulinglargine \\
630 &0.0112 &acetylsalicylicacid metoprolol    &53 &0.0153 &acetylsalicylicacid metformin      &3199 &0.0085 &insulinglargine insulinlispro    &21 &0.0061 &\textbf{lamivudine} lopinavir \\


	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/drug_freq_pair_all.tex <==
\begin{table*}[!h]
  \centering
  \caption{ pair drug frequency of  all  }
  \label{table:perfcmp}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{
	%p{10mm}|p{10mm}|p{10mm}|p{10mm}|p{10mm}|p{10mm}|p{10mm}|p{10mm}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
        @{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
        @{\hspace{2pt}}p{0.15\textwidth}@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
	%@{\hspace{2pt}}l@{\hspace{2pt}}
        %@{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
values & percent & M freq &values&percent & M uniq &values& percent&N freq &values& percent&N uniq \\
	%&M freq	& M uniq &N freq &N uniq \\% 
        \hline
2923 &0.0450 &acetylsalicylicacid \textbf{simvastatin}         &1545 &0.0564 &acetylsalicylicacid \textbf{simvastatin}         &37449 &0.0254 &fluticasonepropionate salmeterol        &21210 &0.0341 &acetaminophen hydrocodone \\
2635 &0.0406 &acetylsalicylicacid \textbf{atorvastatin}        &1458 &0.0532 &acetylsalicylicacid \textbf{atorvastatin}        &37002 &0.0251 &acetaminophen hydrocodone       &18940 &0.0305 &acetylsalicylicacid furosemide \\
2385 &0.0368 &acetaminophen hydrocodone        &1428 &0.0521 &acetaminophen hydrocodone        &27184 &0.0184 &acetylsalicylicacid \textbf{simvastatin}        &18164 &0.0292 &acetylsalicylicacid \textbf{simvastatin} \\
1852 &0.0285 &\textbf{ezetimibe} \textbf{simvastatin}  &1151 &0.0420 &acetylsalicylicacid metoprolol   &26603 &0.0180 &acetylsalicylicacid \textbf{atorvastatin}       &17580 &0.0283 &acetylsalicylicacid metoprolol \\
1832 &0.0282 &acetylsalicylicacid metoprolol   &1119 &0.0409 &acetylsalicylicacid furosemide   &26450 &0.0179 &acetylsalicylicacid clopidogrel         &17499 &0.0282 &fluticasonepropionate salmeterol \\
1757 &0.0271 &acetylsalicylicacid clopidogrel  &1087 &0.0397 &acetylsalicylicacid clopidogrel  &26235 &0.0178 &acetylsalicylicacid furosemide  &17390 &0.0280 &acetylsalicylicacid \textbf{atorvastatin} \\
1698 &0.0262 &acetylsalicylicacid furosemide   &967 &0.0353 &acetaminophen acetylsalicylicacid         &24499 &0.0166 &acetylsalicylicacid metoprolol  &15876 &0.0255 &acetylsalicylicacid clopidogrel \\
1539 &0.0237 &acetylsalicylicacid amlodipine   &906 &0.0331 &acetaminophen oxycodone   &21169 &0.0143 &acetaminophen oxycodone         &13457 &0.0217 &acetylsalicylicacid metformin \\
1530 &0.0236 &acetaminophen acetylsalicylicacid        &896 &0.0327 &acetylsalicylicacid lisinopril    &19930 &0.0135 &exenatide metformin     &13301 &0.0214 &acetylsalicylicacid lisinopril \\
1528 &0.0235 &acetaminophen oxycodone  &862 &0.0315 &acetylsalicylicacid amlodipine    &19810 &0.0134 &conjugatedestrogens medroxyprogesterone         &13028 &0.0210 &acetylsalicylicacid amlodipine \\
1525 &0.0235 &fluticasonepropionate salmeterol         &843 &0.0308 &fluticasonepropionate salmeterol  &19476 &0.0132 &acetylsalicylicacid metformin   &12997 &0.0209 &acetaminophen acetylsalicylicacid \\
1325 &0.0204 &acetylsalicylicacid lisinopril   &822 &0.0300 &acetylsalicylicacid levothyroxine         &19209 &0.0130 &acetaminophen acetylsalicylicacid       &12744 &0.0205 &acetaminophen oxycodone \\
1253 &0.0193 &acetylsalicylicacid levothyroxine        &778 &0.0284 &acetylsalicylicacid \textbf{rosuvastatin}         &19160 &0.0130 &acetylsalicylicacid amlodipine  &11665 &0.0188 &furosemide warfarin \\
1244 &0.0192 &acetylsalicylicacid \textbf{rosuvastatin}        &751 &0.0274 &acetylsalicylicacid metformin     &18781 &0.0127 &metformin rosiglitazone         &11661 &0.0188 &acetylsalicylicacid levothyroxine \\
1194 &0.0184 &amlodipine \textbf{atorvastatin}         &743 &0.0271 &acetylsalicylicacid hydrochlorothiazide   &18773 &0.0127 &fluticasonepropionate salbutamol        &11584 &0.0186 &furosemide potassiumchloride \\
1175 &0.0181 &furosemide \textbf{simvastatin}  &730 &0.0267 &furosemide \textbf{simvastatin}   &18472 &0.0125 &acetylsalicylicacid lisinopril  &10952 &0.0176 &fluticasonepropionate salbutamol \\
1168 &0.0180 &acetylsalicylicacid atenolol     &696 &0.0254 &metoprolol \textbf{simvastatin}   &17004 &0.0115 &sulfamethoxazole trimethoprim   &10633 &0.0171 &acetylsalicylicacid omeprazole \\
1150 &0.0177 &metoprolol \textbf{simvastatin}  &693 &0.0253 &acetylsalicylicacid atenolol      &16843 &0.0114 &salbutamol salmeterol   &10209 &0.0164 &sulfamethoxazole trimethoprim \\
1121 &0.0173 &acetylsalicylicacid metformin    &689 &0.0252 &\textbf{ezetimibe} \textbf{simvastatin}   &16534 &0.0112 &ethinylestradiol norelgestromin         &10204 &0.0164 &furosemide metoprolol \\
1107 &0.0171 &acetylsalicylicacid omeprazole   &685 &0.0250 &acetaminophen furosemide  &16235 &0.0110 &furosemide warfarin     &10089 &0.0162 &acetaminophen furosemide \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_4000.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset $\mathcal{D}^{{4000}}$ wrong SVM}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
        Accuracy	& 0.8730     			& 0.8773     			& 0.8732			& 0.8800			& 0.8715			
			& 0.8630			& 0.7717			& 0.8018			& 0.8677			& 0.8705			\\
        Precision       & 0.9489     			& 0.9365     			& 0.9485			& 0.9364			& 0.9471			
			& 0.8812			& 0.8718			& 0.8401			& 0.9598			& 0.9521			\\
	Recall		& 0.7885     			& 0.8095     			& 0.7895			& 0.8155			& 0.7870			
			& 0.8395			& 0.6370			& 0.7555			& 0.7680			& 0.7805			\\
	F1		& 0.8612     			& 0.8683     			& 0.8616			& 0.8717			& 0.8594			
			& 0.8597			& 0.7360			& 0.7917			& 0.8529			& 0.8576			\\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  some footnotes go here.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_4000_recall_wrong_RBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{Recall from  $\mathcal{D}^{{4000}}$ wrong RBF}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
		 Recall A & 0.9360	& 0.9360	& 0.9350	& 0.9350	& 0.9460	& 0.9100	& 0.8590	& 0.8440	& 0.8950	& 0.9520	\\
		 Recall B & 0.9570	& 0.9570	& 0.9630	& 0.9560	& 0.9580	& 0.9110	& 0.8570	& 0.8250	& 0.9380	& 0.9700	\\
		 Recall C & 0.7250	& 0.7500	& 0.7340	& 0.7520	& 0.7220	& 0.7630	& 0.6800	& 0.7200	& 0.8070	& 0.7010	\\
		 Recall D & 0.9220	& 0.9260	& 0.9180	& 0.9310	& 0.9070	& 0.9230	& 0.8330	& 0.8890	& 0.9750	& 0.9110	\\

        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  some footnotes go here.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_4000_right_with_BBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset $\mathcal{D}^{{4000}}$ RIGHT }
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
 	Accuracy	 & 0.8850 & 0.8923 & 0.8875 & 0.8935 & 0.8832 & 0.8768 & 0.8072 & 0.8195 & 0.8842 & 0.8853 \\
 	Precision        & 0.9390 & 0.9401 & 0.9419 & 0.9392 & 0.9444 & 0.9042 & 0.8419 & 0.8341 & 0.8833 & 0.9539 \\
 	Recall		 & 0.8235 & 0.8380 & 0.8260 & 0.8415 & 0.8145 & 0.8430 & 0.7565 & 0.8045 & 0.8855 & 0.8100 \\
 	F1		 & 0.8775 & 0.8861 & 0.8802 & 0.8877 & 0.8747 & 0.8725 & 0.7969 & 0.8190 & 0.8844 & 0.8761 \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  best gamma in RBF 1st is 1, best gamma in RBF 2nd is 0.1
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_4000_wrong_RBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset $\mathcal{D}^{{4000}}$ Wrong RBF}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
	Accuracy	 & 0.8850 & 0.8923 & 0.8875 & 0.8935 & 0.8832 & 0.8768 & 0.8072 & 0.8195 & 0.9037 & 0.8835	\\
	Precision        & 0.9390 & 0.9401 & 0.9419 & 0.9392 & 0.9444 & 0.9042 & 0.8419 & 0.8341 & 0.9144 & 0.9542	\\
	Recall		 & 0.8235 & 0.8380 & 0.8260 & 0.8415 & 0.8145 & 0.8430 & 0.7565 & 0.8045 & 0.8910 & 0.8060	\\
	F1		 & 0.8775 & 0.8861 & 0.8802 & 0.8877 & 0.8747 & 0.8725 & 0.7969 & 0.8190 & 0.9025 & 0.8739	\\

        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  best gamma in RBF 1st is 1, best gamma in RBF 2nd is 0.1
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_6928.tex <==
\begin{table*}[!h]
  \centering
  \caption{ABCD 6928 instance this is wrong kernel right SVM currently working on it }
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
	%		2dGMgd  coSimGMgd  2dGMop  coSimGMop  2davg   coSimavg  2dProb  coSimProb  rbf1st  rbf2nd
 	Accuracy X	&0.8148	&0.8227    &0.8158 &0.8239    &0.8202 &0.8176   &0.7305 &0.7495    &0.8321 &0.8154\\ 
 	Precision X     &0.9029 &0.8976    &0.9035 &0.8962    &0.9008 &0.8507   &0.8590 &0.7773    &0.8480 &0.9148\\ 
 	Recall	X	&0.7056 &0.7284    &0.7073 &0.7327    &0.7194 &0.7702   &0.5517 &0.6992    &0.8092 &0.6955\\ 
 	F1	X	&0.7921 &0.8042    &0.7935 &0.8062    &0.7999 &0.8085   &0.6719 &0.7362    &0.8281 &0.7902\\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  some footnotes go here.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_6928_recall_wrong_RBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{Recall from  $\mathcal{D}^{{6928}}$Wrong RBF }
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
 		Recall A & 0.8905        & 0.8991        & 0.8941 & 0.8995 & 0.9023 & 0.8723 & 0.8345 & 0.7700 & 0.8686 & 0.9264 \\
 		Recall B & 0.9233        & 0.9209        & 0.9256 & 0.9209 & 0.9248 & 0.8940 & 0.8441 & 0.7832 & 0.9146 & 0.9509 \\
 		Recall C & 0.6810        & 0.6964        & 0.6830 & 0.6993 & 0.6741 & 0.7090 & 0.6303 & 0.7029 & 0.7386 & 0.6120 \\
 		Recall D & 0.9210        & 0.9220        & 0.9230 & 0.9250 & 0.9170 & 0.9190 & 0.8320 & 0.8850 & 0.9710 & 0.9010 \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  some footnotes go here.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_6928_right_with_RBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{ Performance comparison in Dataset $\mathcal{D}^{{6928}}$ right }
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
	%		2dGMgd  coSimGMgd  2dGMop  coSimGMop  2davg   coSimavg  2dProb  coSimProb  rbf1st  rbf2nd
 	Accuracy 	& 0.8264 & 0.8343 & 0.8290 & 0.8359 & 0.8274 & 0.8249 & 0.7633 & 0.7652 & 0.8359 & 0.8274 \\
 	Precision 	& 0.8849 & 0.8912 & 0.8885 & 0.8919 & 0.8926 & 0.8653 & 0.8095 & 0.7704 & 0.8554 & 0.9069 \\
 	Recall		& 0.7503 & 0.7616 & 0.7523 & 0.7645 & 0.7442 & 0.7697 & 0.6885 & 0.7555 & 0.8083 & 0.7295 \\
 	F1 		& 0.8121 & 0.8213 & 0.8147 & 0.8233 & 0.8117 & 0.8147 & 0.7441 & 0.7629 & 0.8312 & 0.8086 \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  best gamma in RBF 1st is 1, best gamma in RBF 2nd is 0.1
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_ABCD_6928_wrong_RBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{ Performance comparison in Dataset $\mathcal{D}^{{6928}}$ wrong rbf}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
	%		2dGMgd  coSimGMgd  2dGMop  coSimGMop  2davg   coSimavg  2dProb  coSimProb  rbf1st  rbf2nd
 	Accuracy 	& 0.8264 & 0.8343 & 0.8290 & 0.8359 & 0.8274 & 0.8249 & 0.7633 & 0.7652 & 0.8456 & 0.8154 \\
	Precision 	& 0.8849 & 0.8912 & 0.8885 & 0.8919 & 0.8926 & 0.8653 & 0.8095 & 0.7704 & 0.8754 & 0.9148 \\
	Recall		& 0.7503 & 0.7616 & 0.7523 & 0.7645 & 0.7442 & 0.7697 & 0.6885 & 0.7555 & 0.8057 & 0.6955 \\
	F1 		& 0.8121 & 0.8213 & 0.8147 & 0.8233 & 0.8117 & 0.8147 & 0.7441 & 0.7629 & 0.8391 & 0.7902 \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  best gamma in RBF 1st is 1, best gamma in RBF 2nd is 0.1
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_AD_2000.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset $\mathcal{D}^{{2000}}$ wrong SVM}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
        Accuracy	& 0.9250     			& 0.9250     			& 0.9240			& 0.9260			& 0.9125					
			& 0.8980			& 0.8340			& 0.8470 			& 0.8805			& 0.9125				\\
        Precision       & 0.9604    			& 0.9490     			& 0.9573			& 0.9490			& 0.9590		
			& 0.8959			& 0.8546			& 0.8595			& 0.8222			& 0.9512				\\
	Recall		& 0.8870     			& 0.8990     			& 0.8880			& 0.9010			& 0.8620		
			& 0.9010			& 0.8050			& 0.8400			& 0.9710			& 0.8700				\\
	F1		& 0.9220     			& 0.9230     			& 0.9211			& 0.9241			& 0.9077		
			& 0.8982			& 0.8286			& 0.8439			& 0.8904			& 0.9086				\\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  some footnotes go here.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_AD_2000_recall_wrong_RBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{Recall from  $\mathcal{D}^{{2000}}$ BC are calculated by average prediction value wrong RBF}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
		 Recall A  & 0.9580	& 0.9610	& 0.9560	& 0.9600	& 0.9600 & 0.9170	& 0.8360	& 0.8510	& 0.8750	& 0.9610	\\
		 Recall B  & 0.9730	& 0.9740	& 0.9740	& 0.9780	& 0.9750 & 0.9160	& 0.8420	& 0.7980	& 0.9270	& 0.9820	\\
		 Recall C  & 0.5860	& 0.5010	& 0.5870	& 0.5100	& 0.6290 & 0.6900	& 0.6360	& 0.6900	& 0.6170	& 0.5290	\\
		 Recall D  & 0.9020	& 0.9100	& 0.9020	& 0.9160	& 0.8880 & 0.9070	& 0.8540	& 0.8690	& 0.9640	& 0.8810	\\

        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  some footnotes go here.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_AD_2000_right_with_BRF.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset $\mathcal{D}^{{2000}}$ RIGHT}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline






 		 Accuracy	& 0.9300 & 0.9355 & 0.9290 & 0.9380 & 0.9240 & 0.9120 & 0.8450 & 0.8600 & 0.9250 & 0.9195 \\
 		 Precision      & 0.9560 & 0.9593 & 0.9540 & 0.9585 & 0.9571 & 0.9166 & 0.8391 & 0.8595 & 0.9674 & 0.9559 \\
 		 Recall		& 0.9020 & 0.9100 & 0.9020 & 0.9160 & 0.8880 & 0.9070 & 0.8540 & 0.8690 & 0.8800 & 0.8800 \\
 		 F1		& 0.9282 & 0.9340 & 0.9273 & 0.9368 & 0.9213 & 0.9118 & 0.8465 & 0.8642 & 0.9216 & 0.9164 \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  best gamma in RBF 1st is 0.1, best gamma in RBF 2nd is 0.1
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_AD_2000_wrong_RBF.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset $\mathcal{D}^{{2000}}$ Wrong RBF} 
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
		 Accuracy	& 0.9300 & 0.9355 & 0.9290 & 0.9380 & 0.9240 & 0.9120 & 0.8450 & 0.8600 & 0.9195 & 0.9210	\\
		 Precision      & 0.9560 & 0.9593 & 0.9540 & 0.9585 & 0.9571 & 0.9166 & 0.8391 & 0.8595 & 0.8854 & 0.9581	\\
		 Recall		& 0.9020 & 0.9100 & 0.9020 & 0.9160 & 0.8880 & 0.9070 & 0.8540 & 0.8690 & 0.9640 & 0.8810	\\
		 F1		& 0.9282 & 0.9340 & 0.9273 & 0.9368 & 0.9213 & 0.9118 & 0.8465 & 0.8642 & 0.9230 & 0.9179	\\

        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  best gamma in RBF 1st is 1, best gamma in RBF 2nd is 0.1
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/results_AD_3200.tex <==
\begin{table*}[!h]
  \centering
  \caption{ABCD 3200 instance}
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	}
        \hline\hline
			& $\mathcal{K}^{2d}_{GMgd}$ 	& $\mathcal{K}^{coSim}_{GMgd}$	& $\mathcal{K}^{2d}_{GMop}$ 	& $\mathcal{K}^{coSim}_{GMop}$	& $\mathcal{K}^{2d}_{avg}$	
			& $\mathcal{K}^{coSim}_{avg}$	& $\mathcal{K}^{2d}_{prob}$	& $\mathcal{K}^{coSim}_{prob}$	& $\mathcal{K}^{1st}_{rbf}$   	& $\mathcal{K}^{2nd}_{rbf}$		\\
        \hline
        Accuracy	&      			&      			& 			& 			& 			
			& 			& 			& 			& 			& 			\\
        Precision       &      			&      			& 			& 			& 			
			& 			& 			& 			& 			& 			\\
	Recall		&      			&      			& 			& 			& 			
			& 			& 			& 			& 			& 			\\
	F1		&      			&      			& 			& 			& 			
			& 			& 			& 			& 			& 			\\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  some footnotes go here.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/top_prediction_combinations_D2000.tex <==
\begin{table*}[!h]
  \centering
  \caption{top prediction value combinations in \GMop of \DIIk }
  \label{table:top_com_d2k}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
	@{\hspace{0pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}   
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
	N	& prd &frq	& Combinations		\\
        \hline
1 &3.064 & 3 &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}   \\
2 &2.784 & 9 &\textbf{atorvastatin} \textbf{fenofibrate} \textbf{pravastatin} \textbf{simvastatin}   \\
3 &2.755 & 5 &\textbf{atorvastatin} fluconazole levothyroxine \textbf{simvastatin}   \\
4 &2.747 & 11&\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{simvastatin}   \\
5 &2.602 & 6 &\textbf{atorvastatin} celecoxib escitalopram gabapentin levofloxacin levothyroxine liothyronine risedronate \textbf{simvastatin}   \\
6 &2.528 & 4 &alprazolam \textbf{atorvastatin} imipramine levothyroxine \textbf{simvastatin}   \\
7 &2.504 & 6 &\textbf{atorvastatin} fexofenadine fluticasonepropionate levofloxacin nitrofurantoin \textbf{simvastatin}   \\
8 &2.452 & 4 &\textbf{allopurinol} \textbf{amiodarone} \textbf{atorvastatin} furosemide omeprazole \textbf{simvastatin}   \\
9 &2.420 & 13&\textbf{atorvastatin} esomeprazole hydrochlorothiazide losartan potassium ramipril \textbf{simvastatin}   \\
10&2.416 & 5 &acetylsalicylicacid lansoprazole lisinopril \textbf{pravastatin} quinine \textbf{simvastatin}   \\
		

	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	 Prediction values and frequency are denoted as prd and frq, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/top_prediction_combinations_D2000_miss_classi.tex <==
\begin{table*}[!h]
  \centering
  \caption{top prediction value combinations in \GMop of \DIIk with negative label miss classification }
  \label{table:top_com_d2k_miss}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
        @{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	}
        \hline\hline
	N       & prd &frq      & Combinations          \\
        \hline
1&1.565  & 58 &acetylsalicylicacid \textbf{amiodarone} bisoprolol digoxin \textbf{ezetimibe} furosemide lansoprazole perindopril  \\
2&1.441  & 38 &ramipril ranitidine \textbf{simvastatin}  \\
3&1.438  & 33 &acetylsalicylicacid \textbf{amiodarone} bisoprolol digoxin \textbf{ezetimibe} furosemide lansoprazole perindopril warfarin  \\
4&1.312  & 35 &\textbf{aripiprazole} \textbf{atorvastatin} bendroflumethiazide clozapine diazepam folicacid furosemide iron lactulose lansoprazole perindopril ramipril trimethoprim \textbf{zopiclone}  \\
5&1.296  & 38 &acetaminophen amlodipine \textbf{citalopram} codeine diazepam doxazosin perindopril temazepam  \\
6&1.281  & 40 &\textbf{atorvastatin} formoterol furosemide metformin prednisolone ramipril salbutamol verapamil warfarin  \\
7&1.239  & 41 &acetaminophen acetylsalicylicacid \textbf{atorvastatin} bendroflumethiazide doxycycline furosemide metformin oxycodone \textbf{pregabalin} ramipril  \\
8&1.180  & 40 &\textbf{allopurinol} cetirizine \textbf{colchicine} doxazosin metformin mirtazapine valsartan  \\
9&0.992  & 48 &finasteride lamotrigine latanoprost levothyroxine ramipril tamsulosin warfarin  \\
10&0.975 & 36 &acyclovir ciprofloxacin itraconazole methotrexate omeprazole tacrolimus  \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  Prediction values and frequency are denoted as prd and frq, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/top_prediction_combinations_D2000_without_Myo_drugs.tex <==
\begin{table*}[!h]
  \centering
  \caption{ top prediction value combinations in \GMop of \DIIk without Myopathy self-induced drug }
  \label{table:top_com_d2k_without_M}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
@{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	}
        \hline\hline
	N       & prd &frq      & Combinations          \\
        \hline
1 &1.947 &4 &acetylsalicylicacid amlodipine bisoprolol lorazepam omeprazole  \\
2 &1.857 &7 &acyclovir amlodipine cephalexin folicacid losartan mirtazapine potassium ranitidine trimethoprim  \\
3 &1.850 &7 &alendronate cyclobenzaprine meloxicam potassiumchloride triamterene vitamine  \\
4 &1.832 &4 &azithromycin diazepam drospirenone ibuprofen levothyroxine mometasone  \\
5 &1.819 &5 &famotidine levothyroxine metoprolol nadolol tamsulosin telmisartan  \\
6 &1.795 &4 &calcium clonazepam colestipol prednisone teriparatide  \\
7 &1.794 &5 &carisoprodol clonidine duloxetine furosemide gabapentin losartan metoprolol morphine norethindrone nortriptyline omeprazole potassiumchloride  \\
8 &1.776 &5 &alendronate fexofenadine levothyroxine nabumetone oxybutynin  \\
9 &1.757 &6 &acetaminophen alendronate amitriptyline ibandronate lansoprazole opoxyphene vitamine  \\
10&1.752 &5 &alprazolam esomeprazole lansoprazole naproxen omeprazole prednisone  \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	 Prediction values and frequency are denoted as prd and frq, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/top_prediction_combinations_D4000.tex <==
\begin{table*}[!h]
  \centering
  \caption{ top prediction value combinations in \GMop of \DIVk  }
  \label{table:top_com_d4k}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{10mm}|p{100mm}
        @{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{8pt}}l@{\hspace{8pt}}
	}
        \hline\hline
		N	& prd	& frq &OR & Combinations		\\
        \hline


1 &4.291 & 3  &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
2 &3.954 & -  & 140.9700&\textbf{atorvastatin} \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin} tadalafil  \\
3 &3.948 & -  & 52.0340 &\textbf{atorvastatin} \textbf{fenofibrate} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
4 &3.881 & -  & 83.2800 &\textbf{atorvastatin} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
5 &3.797 & -  & 18.8940 &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{rosuvastatin} \textbf{simvastatin}  \\
6 &3.726 & 10 &  -      &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{fenofibrate} \textbf{rosuvastatin}  \\
7 &3.557 & 9  &  -      &\textbf{atorvastatin} \textbf{fenofibrate} \textbf{pravastatin} \textbf{simvastatin}  \\
8 &3.518 & 11 &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{simvastatin}  \\
9 &3.496 & -  & 11.6710 &\textbf{atorvastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
10&3.422 & 6  &  -      &\textbf{atorvastatin} celecoxib escitalopram gabapentin levofloxacin levothyroxine liothyronine risedronate \textbf{simvastatin}  \\

        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  Prediction values, frequency and odds ratio are denoted as prd, frq and OR, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/top_prediction_combinations_D4000_miss_classi.tex <==
\begin{table*}[!h]
  \centering
  \caption{ top prediction value combinations in \GMop of \DIVk with negative label miss classification  }
  \label{table:top_com_d4k_miss}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
        @{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	}
        \hline\hline
N       & prd   & frq &OR & Combinations                \\
        \hline
 1      &1.756 & 35 & -      &\textbf{aripiprazole} \textbf{atorvastatin} bendroflumethiazide clozapine diazepam folicacid furosemide iron lactulose lansoprazole perindopril ramipril trimethoprim \textbf{zopiclone}  \\
 2      &1.624 & 38 & -      &ramipril ranitidine \textbf{simvastatin}  \\
 3      &1.603 & 41 & -      &acetaminophen acetylsalicylicacid \textbf{atorvastatin} bendroflumethiazide doxycycline furosemide metformin oxycodone \textbf{pregabalin} ramipril  \\
 4      &1.526 & 58 & -      &acetylsalicylicacid \textbf{amiodarone} bisoprolol digoxin \textbf{ezetimibe} furosemide lansoprazole perindopril  \\
 5      &1.480 & 35 & -      &\textbf{ezetimibe} \textbf{simvastatin} varenicline  \\
 6      &1.474 & 38 & -      &acetaminophen amlodipine \textbf{citalopram} codeine diazepam doxazosin perindopril temazepam  \\
 7      &1.368 & 33 & -      &acetylsalicylicacid \textbf{amiodarone} bisoprolol digoxin \textbf{ezetimibe} furosemide lansoprazole perindopril warfarin  \\
 8      &1.354 &  - & 0.6953 &acetylsalicylicacid \textbf{ezetimibe} \textbf{niacin} \textbf{simvastatin}  \\
 9      &1.044 & 38 & -      &acetylsalicylicacid dipyridamole \textbf{simvastatin}  \\
 10     &1.000 &  - & 0.4134 &alendronate ibandronate zoledronate  \\


        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  Prediction values, frequency and odds ratio are denoted as prd, frq and OR, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/top_prediction_combinations_D4000_without_Myo_drugs.tex <==
\begin{table*}[!h]
  \centering
  \caption{ top prediction value combinations in \GMop of \DIVk without Myopathy self-induced drug  }
  \label{table:top_com_d4k_without_M}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{10mm}|p{100mm}
	@{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	}	
        \hline\hline
		N       & prd   & frq &OR & Combinations                \\
        \hline
1 &2.264  &4 &- &calcium clonazepam colestipol prednisone teriparatide  \\
2 &2.226  &- &108.5500 &alendronate amlodipine atenolol clonazepam raloxifene teriparatide  \\
3 &2.025  &- &132.1900 &alendronate calcium esomeprazole ibandronate levothyroxine rabeprazole  \\
4 &2.009  &7 &- &alendronate cyclobenzaprine meloxicam potassiumchloride triamterene vitamine  \\
5 &1.999  &- &37.4830 &alitretinoin clindamycin doxycycline erythromycin ethinylestradiol lansoprazole metronidazole minocycline norgestimate sulfamethoxazole tretinoin trimethoprim  \\
6 &1.983  &5 &- &alendronate fexofenadine levothyroxine nabumetone oxybutynin  \\
7 &1.943  &- &11.0220 &alendronate calcium cholecalciferol omeprazole vitaminc  \\
8 &1.935  &6 &- &acetaminophen alendronate amitriptyline ibandronate lansoprazole opoxyphene vitamine  \\
9 &1.838  &- &53.2870 &ethinylestradiol etonogestrel loratadine omeprazole sertraline topiramate  \\
10&1.828  &4 &- &acetaminophen alendronate desloratadine diphenhydramine fexofenadine loratadine  \\         
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  Prediction values, frequency and odds ratio are denoted as prd, frq and OR, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups/top_prediction_combinations_D6928.tex <==
\begin{table*}[!h]
  \centering
  \caption{top prediction values in different Kernel $\mathcal{D}^{{6928}}$ }
  \label{table:perfcmp}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}
	{p{10mm}|p{10mm}|p{150mm}
	@{\hspace{8pt}}l@{\hspace{10pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}          
	@{\hspace{8pt}}l@{\hspace{8pt}}
	}
        \hline\hline
		Kernel				& top prediction value	& Combinations		\\
        \hline
		$\mathcal{K}^{2d}_{GMgd}$ 	&3.7385 &db00641:simvastatin ; db00710:ibandronate ; db00973:ezetimibe ; db01039:fenofibrate ; db01095:fluvastatin ; db01098:rosuvastatin ; db01432:cholestyramine ;  \newline \\
		$\mathcal{K}^{coSim}_{GMgd}$ 	&3.9561 &db00175:pravastatin ; db00448:lansoprazole ; db00641:simvastatin ; db01076:atorvastatin ; db01098:rosuvastatin ;  \newline \\
		$\mathcal{K}^{2d}_{GMop}$ 	&3.7072 &db00641:simvastatin ; db00710:ibandronate ; db00973:ezetimibe ; db01039:fenofibrate ; db01095:fluvastatin ; db01098:rosuvastatin ; db01432:cholestyramine ;  \newline \\
		$\mathcal{K}^{coSim}_{GMop}$ 	&4.1670 &db00175:pravastatin ; db00448:lansoprazole ; db00641:simvastatin ; db01076:atorvastatin ; db01098:rosuvastatin ;  \newline \\
		$\mathcal{K}^{2d}_{avg}$ 	&\textbf{5.5751} &db00641:simvastatin ; db00710:ibandronate ; db00973:ezetimibe ; db01039:fenofibrate ; db01095:fluvastatin ; db01098:rosuvastatin ; db01432:cholestyramine ;  \newline \\
		$\mathcal{K}^{coSim}_{avg}$ 	&4.4574 &db00175:pravastatin ; db00641:simvastatin ; db01076:atorvastatin ; db01098:rosuvastatin ;  \newline \\
		$\mathcal{K}^{2d}_{prob}$ 	&1.9512 &db00175:pravastatin ; db00448:lansoprazole ; db00641:simvastatin ; db01076:atorvastatin ; db01098:rosuvastatin ;  \newline \\
		$\mathcal{K}^{coSim}_{prob}$     &2.0096 &db00175:pravastatin ; db00448:lansoprazole ; db00641:simvastatin ; db01076:atorvastatin ; db01098:rosuvastatin ;  \newline \\
		$\mathcal{K}^{1st}_{tan}$	&3.7096 &db00175:pravastatin ; db00641:simvastatin ; db01076:atorvastatin ; db01098:rosuvastatin ;  \newline \\
		$\mathcal{K}^{2nd}_{tan}$ 	&2.6228 &db00641:simvastatin ; db01076:atorvastatin ; db01098:rosuvastatin ;  \newline \\
			
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/RTkernel_ABCD_4000.tex <==
\begin{table*}[!h]
  \centering
  \caption{Running time comparison in Dataset \DIVk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{2pt}}c@{\hspace{2pt}}
          %a
          @{\hspace{2pt}}r@{\hspace{1pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
   	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %          
	  @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}          
          @{\hspace{2pt}}r@{\hspace{2pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline


        Kernel          & 5325.9345  & 5453.9561  && 2817.0034 & 3330.7596 && 1003.7010  & 949.8912   && 13690.1682  & 17540.1613  && 0.9258 & 0.5542       \\
        SVM             & 0.8320     & 0.8280     && 0.8420    & 0.8100    && 0.6320     & 0.6360     && 1.3200      & 1.2940      && 0.7600 & 0.8580       \\



        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/RTkernel_ABCD_6928.tex <==
\begin{table*}[!h]
  \centering
  \caption{Running time comparison in Dataset \DVIk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{2pt}}c@{\hspace{2pt}}
          %a
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
   	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %          
	  @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}          
          @{\hspace{2pt}}r@{\hspace{2pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline

        Kernel          & 16588.9441 & 25317.1467 && 8876.1919 & 10163.9581  && 2360.9811     & 4666.4940     && 58354.0316    & 53583.0757    && 0.6850        & 0.7683\\
        SVM             & 3.6900     & 4.2500     && 3.6820    & 3.8240      && 1.6240        & 1.8800        && 6.7360        & 6.7040        && 5.6720        & 4.6740\\



        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/RTkernel_AD_2000.tex <==
\begin{table*}[!h]
  \centering
  \caption{ Running time comparison in Dataset \DIIk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{2pt}}l@{\hspace{2pt}}
          %a
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
   	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %          
	  @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
	  @{\hspace{2pt}}r@{\hspace{2pt}}
	  %
          @{\hspace{2pt}}r@{\hspace{2pt}}          
          @{\hspace{2pt}}r@{\hspace{2pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline
        Kernel          & 1577.7462  & 1505.2766  && 728.0588  & 924.6410  && 259.4984   & 277.1828    && 7219.7460   & 7183.8025   && 0.1840 & 0.2260      \\
        SVM             & 0.1760     & 0.1920     && 0.1540    & 0.1840    && 0.1740     & 0.1800      && 0.3600      & 0.3380      && 0.1784 & 0.2239      \\




        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/results_ABCD_4000.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset \DIVk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{8pt}}l@{\hspace{10pt}}
          %a
          @{\hspace{8pt}}c@{\hspace{10pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
   	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %          
	  @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}          
          @{\hspace{8pt}}c@{\hspace{8pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline

        Accuracy         & 0.8850 & 0.8923 && 0.8875 & \textbf{0.8935}  && 0.8832               & 0.8768                && 0.8072 & 0.8195 && 0.8695 & 0.8808 \\
        Precision        & 0.9390 & 0.9401 && 0.9419 & 0.9392           && \textbf{0.9444}      & 0.9042                && 0.8419 & 0.8341 && 0.9328 & 0.9341 \\
        Recall           & 0.8235 & 0.8380 && 0.8260 & 0.8415           && 0.8145               & \textbf{0.8430}       && 0.7565 & 0.8045 && 0.7965 & 0.8195 \\
        F1               & 0.8775 & 0.8861 && 0.8802 & \textbf{0.8877}  && 0.8747               & 0.8725                && 0.7969 & 0.8190 && 0.8593 & 0.8731 \\
        AUC              & 0.9476 & 0.9553 && 0.9474 & \textbf{0.9573}  && 0.9484               & 0.9418                && 0.8938 & 0.9014 && 0.9530 & 0.9553 \\


        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/results_ABCD_4000_precision_4.tex <==
\begin{table}[!h]
  \centering
  \caption{Performance comparison in Dataset \DIVk}
  \label{table:result_4k}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{1pt}}l@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          %
        }
        \hline\hline
	& \multicolumn{2}{c}{\GMop}   && \multicolumn{2}{c}{\GMtan}   && \multicolumn{2}{c}{\GMavg}   && \multicolumn{2}{c}{\GMprob} \\
				   %& \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
\cline{2-3}                 \cline{5-6}                 \cline{8-9}                  \cline{11-12}
	& \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline
Acc & 0.8875 & \textbf{0.8935}  && 0.8695 & 0.8808	&& 0.8832               & 0.8768                && 0.8072 & 0.8195  \\
Pre & 0.9419 & 0.9392           && 0.9328 & 0.9341	&& \textbf{0.9444}      & 0.9042                && 0.8419 & 0.8341  \\
Rec & 0.8260 & 0.8415           && 0.7965 & 0.8195	&& 0.8145               & \textbf{0.8430}       && 0.7565 & 0.8045  \\
F1  & 0.8802 & \textbf{0.8877}  && 0.8593 & 0.8731	&& 0.8747               & 0.8725                && 0.7969 & 0.8190  \\
AUC & 0.9474 & \textbf{0.9573}  && 0.9530 & 0.9553	&& 0.9484               & 0.9418                && 0.8938 & 0.9014  \\

        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		Accuracy, precision, recall, and area under the curve of receiver operating characteristic curve is denoted as Acc, Pre, Rec, and AUC, respectively.

          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table}
%


==> results_table/back_ups_old_format/results_ABCD_4000_recall.tex <==
\begin{table*}[!h]
  \centering
  \caption{Recall Performance comparison in Dataset \DIVk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{8pt}}c@{\hspace{10pt}}
          %a
          @{\hspace{8pt}}c@{\hspace{10pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
   	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %          
	  @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}          
          @{\hspace{8pt}}c@{\hspace{8pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline

    Recall A  & 0.9360        & 0.9360        &&  0.9350      		& 0.9350        	&& \textbf{0.9460}      & 0.9100        	&& 0.8590        & 0.8440      && 0.9420 & 0.9390    \\
    Recall B  & 0.9570        & 0.9570        &&  \textbf{0.9630}       & 0.9560        	&& 0.9580        	& 0.9110        	&& 0.8570        & 0.8250      && 0.9430 & 0.9450    \\
    Recall C  & 0.7250        & 0.7500        &&  0.7340       		& 0.7520        	&& 0.7220        	& \textbf{0.7630}       && 0.6800        & 0.7200      && 0.7250 & 0.7430    \\
    Recall D  & 0.9220        & 0.9260        &&  0.9180       		& \textbf{0.9310}       && 0.9070        	& 0.9230        	&& 0.8330        & 0.8890      && 0.8680 & 0.8960    \\



        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/results_ABCD_6928.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset \DVIk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{8pt}}l@{\hspace{10pt}}
          %a
          @{\hspace{8pt}}c@{\hspace{10pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
   	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %          
	  @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}          
          @{\hspace{8pt}}c@{\hspace{8pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline

        Accuracy        & 0.8264 & 0.8343 && 0.8290 & \textbf{0.8359}   && 0.8274               & 0.8249                && 0.7633 & 0.7652 && 0.8171 & 0.8270 \\
        Precision       & 0.8849 & 0.8912 && 0.8885 & 0.8919            && \textbf{0.8926}      & 0.8653                && 0.8095 & 0.7704 && 0.8791 & 0.8781 \\
        Recall          & 0.7503 & 0.7616 && 0.7523 & 0.7645            && 0.7442               & \textbf{0.7697}       && 0.6885 & 0.7555 && 0.7353 & 0.7593 \\
        F1              & 0.8121 & 0.8213 && 0.8147 & \textbf{0.8233}   && 0.8117               & 0.8147                && 0.7441 & 0.7629 && 0.8008 & 0.8144 \\
        AUC             & 0.8971 & 0.9083 && 0.8978 & \textbf{0.9115}   && 0.8995               & 0.8998                && 0.8425 & 0.8525 && 0.9068 & 0.9092 \\



        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/results_ABCD_6928_precision_4.tex <==
\begin{table}[!h]
  \centering
  \caption{Performance comparison in Dataset \DVIk}
  \label{table:result_6k}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{1pt}}l@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
         %
        }
        \hline\hline
& \multicolumn{2}{c}{\GMop}   && \multicolumn{2}{c}{\GMtan}   && \multicolumn{2}{c}{\GMavg}   && \multicolumn{2}{c}{\GMprob} \\
                                   %& \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
\cline{2-3}                 \cline{5-6}                 \cline{8-9}                  \cline{11-12}
        & \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\

	\hline

Acc  & 0.8290 & \textbf{0.8359} && 0.8171 & 0.8270&& 0.8274          & 0.8249          && 0.7633 & 0.7652  \\
Pre  & 0.8885 & 0.8919          && 0.8791 & 0.8781&& \textbf{0.8926} & 0.8653          && 0.8095 & 0.7704  \\
Rec  & 0.7523 & 0.7645          && 0.7353 & 0.7593&& 0.7442          & \textbf{0.7697} && 0.6885 & 0.7555  \\
F1   & 0.8147 & \textbf{0.8233} && 0.8008 & 0.8144&& 0.8117          & 0.8147          && 0.7441 & 0.7629  \\
AUC  & 0.8978 & \textbf{0.9115} && 0.9068 & 0.9092&& 0.8995          & 0.8998          && 0.8425 & 0.8525  \\

        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	Accuracy, precision, recall, and area under the curve of receiver operating characteristic curve is denoted as Acc, Pre, Rec, and AUC, respectively.

          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table}
%


==> results_table/back_ups_old_format/results_ABCD_6928_recall.tex <==
\begin{table*}[!h]
  \centering
  \caption{Recall Performance comparison in Dataset \DVIk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{8pt}}c@{\hspace{10pt}}
          %a
          @{\hspace{8pt}}c@{\hspace{10pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
   	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %          
	  @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}          
          @{\hspace{8pt}}c@{\hspace{8pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline

         Recall A & 0.8905        & 0.8991        && 0.8941        	& 0.8995        	&& \textbf{0.9023}      & 0.8723        	&& 0.8345        & 0.7700 && 0.8945 & 0.8918 \\
         Recall B & 0.9233        & 0.9209        && \textbf{0.9256}    & 0.9209        	&& 0.9248        	& 0.8940        	&& 0.8441        & 0.7832 && 0.9066 & 0.8995 \\
         Recall C & 0.6810        & 0.6964        && 0.6830        	& 0.6993        	&& 0.6741        	& \textbf{0.7090}       && 0.6303        & 0.7029 && 0.6749 & 0.6972 \\
         Recall D & 0.9210        & 0.9220        && 0.9230        	& \textbf{0.9250}       && 0.9170        	& 0.9190        	&& 0.8320        & 0.8850 && 0.8840 & 0.9120 \\


        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/results_AD_2000.tex <==
\begin{table*}[!h]
  \centering
  \caption{Performance comparison in Dataset \DIIk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{8pt}}l@{\hspace{10pt}}
          %a
          @{\hspace{8pt}}c@{\hspace{10pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
   	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %          
	  @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}          
          @{\hspace{8pt}}c@{\hspace{8pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline
                 Accuracy       & 0.9300 & 0.9355 && 0.9290 & \textbf{0.9380} && 0.9240 & 0.9120 && 0.8450 & 0.8600 && 0.8965 & 0.9095 \\
                 Precision      & 0.9560 & 0.9593 && 0.9540 & \textbf{0.9585} && 0.9571 & 0.9166 && 0.8391 & 0.8595 && 0.9407 & 0.9423 \\
                 Recall         & 0.9020 & 0.9100 && 0.9020 & \textbf{0.9160} && 0.8880 & 0.9070 && 0.8540 & 0.8690 && 0.8470 & 0.8730 \\
                 F1             & 0.9282 & 0.9340 && 0.9273 & \textbf{0.9368} && 0.9213 & 0.9118 && 0.8465 & 0.8642 && 0.8914 & 0.9063 \\
                 AUC            & 0.9727 & 0.9756 && 0.9730 & \textbf{0.9761} && 0.9695 & 0.9596 && 0.9195 & 0.9264 && 0.9642 & 0.9675 \\

	
	\hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/back_ups_old_format/results_AD_2000_precision_4.tex <==
\begin{table}[!h]
  \centering
  \caption{Performance comparison in Dataset \DIIk}
  \label{table:result_2k}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{1pt}}l@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
   	  @{\hspace{1pt}}c@{\hspace{0pt}}
	  @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
	  @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}
	  @{\hspace{1pt}}c@{\hspace{0pt}}
          @{\hspace{1pt}}c@{\hspace{0pt}}          
          @{\hspace{1pt}}c@{\hspace{0pt}}
          %
        }
        \hline\hline
	 & \multicolumn{2}{c}{\GMop}	&& \multicolumn{2}{c}{\GMtan}	&& \multicolumn{2}{c}{\GMavg}	&& \multicolumn{2}{c}{\GMprob} \\
				  %& \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12}
	& \IID       & \coSim        && \orderI & \orderII	&& \IID & \coSim	&& \IID & \coSim	\\
	\hline
Acc       & 0.9290 & \textbf{0.9380}&& 0.8965 & 0.9095 && 0.9240 & 0.9120 && 0.8450 & 0.8600  \\
Pre       & 0.9540 & \textbf{0.9585}&& 0.9407 & 0.9423 && 0.9571 & 0.9166 && 0.8391 & 0.8595  \\
Rec       & 0.9020 & \textbf{0.9160}&& 0.8470 & 0.8730 && 0.8880 & 0.9070 && 0.8540 & 0.8690  \\
F1        & 0.9273 & \textbf{0.9368}&& 0.8914 & 0.9063 && 0.9213 & 0.9118 && 0.8465 & 0.8642  \\
AUC       & 0.9730 & \textbf{0.9761}&& 0.9642 & 0.9675 && 0.9695 & 0.9596 && 0.9195 & 0.9264  \\
	
	\hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		Accuracy, precision, recall, and area under the curve of receiver operating characteristic curve is denoted as Acc, Pre, Rec, and AUC, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table}
%


==> results_table/back_ups_old_format/results_AD_2000_recall.tex <==
\begin{table*}[!h]
  \centering
  \caption{Recall Performance comparison in Dataset \DIIk}
  \label{table:perfcmp}
  \begin{threeparttable}
   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{8pt}}l@{\hspace{10pt}}
          %a
          @{\hspace{8pt}}c@{\hspace{10pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
   	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %          
	  @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}
          @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
	  @{\hspace{8pt}}c@{\hspace{8pt}}
	  %
          @{\hspace{8pt}}c@{\hspace{8pt}}          
          @{\hspace{8pt}}c@{\hspace{8pt}}
          %
        }
        \hline\hline
				   & \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12} 	                 \cline{14-15}
				    & \IID & \coSim && \IID & \coSim && \IID & \coSim && \IID & \coSim && \orderI & \orderII \\
	\hline

        Recall A & 0.9580        & \textbf{0.9610}      && 0.9560        & 0.9600        	&& 0.9600        & 0.9170        	&& 0.8360        & 0.8510   		&& 0.9460 & 0.9460      \\
        Recall B & 0.9730        & 0.9740        	&& 0.9740        & \textbf{0.9780}      && 0.9750        & 0.9160        	&& 0.8420        & 0.7980   		&& 0.9650 & 0.9660      \\
        Recall C & 0.5860        & 0.5010        	&& 0.5870        & 0.5100        	&& 0.6290        & \textbf{0.6900}      && 0.6360        & \textbf{0.6900}  	&& 0.6650 & 0.6720      \\
        Recall D & 0.9020        & 0.9100        	&& 0.9020        & \textbf{0.9160}      && 0.8880        & 0.9070       	&& 0.8540        & 0.8690   		&& 0.8470 & 0.8730      \\



        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		footnotes
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> results_table/results_ABCD_4000.tex <==
\begin{table}[t]
  \centering
  \caption{Overall Performance Comparison of \Dfourk}
  \label{table:result_4k}
  \begin{threeparttable}
   %\begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{0pt}}l@{\hspace{3pt}}
          @{\hspace{0pt}}c@{\hspace{0pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{0pt}}         
 %
        }
        \hline\hline
        \multicolumn{1}{c}{$\mathcal{K}$} && \multicolumn{2}{c}{\GMop}   && \multicolumn{2}{c}{\GMtan}   && \multicolumn{2}{c}{\GMavg}   && \multicolumn{2}{c}{\GMprob} \\
                                   %& \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
        \cline{1-1} \cline{3-4}                 \cline{6-7}                 \cline{9-10}                  \cline{12-13}
        ~~\SDS && \IID & \coSim && \orderI & \orderII && \IID & \coSim && \IID & \coSim \\

        \hline 
acc  && 0.888 & \textbf{0.894}  && 0.870 & 0.881  &&  0.883               & 0.877           &&  0.807 & 0.820  \\
pre  && 0.942 & 0.939           && 0.933 & 0.934  &&  \textbf{0.944}      & 0.904           &&  0.842 & 0.834  \\
rec  && 0.826 & 0.842           && 0.797 & 0.820  &&  0.815               & \textbf{0.843}  &&  0.757 & 0.805  \\
F1   && 0.880 & \textbf{0.888}  && 0.859 & 0.873  &&  0.875               & 0.873           &&  0.797 & 0.819  \\
AUC  && 0.947 & \textbf{0.957}  && 0.953 & 0.955  &&  0.948               & 0.942           &&  0.894 & 0.901  \\
	\hline
	\multicolumn{9}{c}{$M zeros$}\\
	\hline
acc  &&  0.896 		&  \textbf{0.899} &&  0.867 &  0.882 &&  0.887  	 &  0.880  &&   &   \\
pre  &&  0.933 		&  0.939 	  &&  0.928 &  0.930 &&  \textbf{0.944}  &  0.903  &&   &   \\
rec  &&  0.853 		&  \textbf{0.854} &&  0.795 &  0.826 &&  0.822  	 &  0.851  &&   &   \\
F1   &&  0.891 		&  \textbf{0.894} &&  0.856 &  0.875 &&  0.879  	 &  0.876  &&   &   \\
AUC  &&  0.953 		&  \textbf{0.962} &&  0.954 &  0.958 &&  0.951  	 &  0.945  &&   &   \\

%        \hline\hline
%	& \multicolumn{2}{c}{\GMop}   && \multicolumn{2}{c}{\GMtan}   && \multicolumn{2}{c}{\GMavg}   && \multicolumn{2}{c}{\GMprob} \\
%				   %& \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
%\cline{2-3}                 \cline{5-6}                 \cline{8-9}                  \cline{11-12}
%	& \IID & \coSim && \orderI & \orderII && \IID & \coSim && \orderI & \orderII \\
%	\hline
%Acc & 0.888 & \textbf{0.894}  && 0.870 & 0.881	&& 0.883               & 0.877                && 0.807 & 0.820  \\
%Pre & 0.942 & 0.939           && 0.933 & 0.934	&& \textbf{0.944}      & 0.904                && 0.842 & 0.834  \\
%Rec & 0.826 & 0.842           && 0.797 & 0.820	&& 0.815               & \textbf{0.843}       && 0.757 & 0.805  \\
%F1  & 0.880 & \textbf{0.888}  && 0.860 & 0.873	&& 0.875               & 0.873                && 0.797 & 0.819  \\
%AUC & 0.947 & \textbf{0.957}  && 0.953 & 0.955	&& 0.948               & 0.942                && 0.894 & 0.901  \\

        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
       In this table, ``acc'', ``pre'', ``rec'' and ``AUC'' represent
        accuracy, precision, recall, and the area under an receiver operating characteristic curve, respectively.
        In \GMtan, ``\orderI'' is the kernel, in which the similarity between two drug combinations is calculated by the feature vectors, whose dimensions correspond to only one drug.
        As for ``\orderII'', the similarity between two drug combinations is calculated by the feature vectors, which have dimensions that correspond to different pairs of drugs.


          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
 %  \end{center}	
  \end{threeparttable}
\end{table}
%


==> results_table/results_ABCD_4000_Mzeros.tex <==
\begin{table}[h]
  \centering
  \caption{Overall Performance Comparison of \Dfourk Mzeros}
  \label{table:result_4k_Mzeros}
  \begin{threeparttable}
   %\begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{0pt}}l@{\hspace{3pt}}
          @{\hspace{0pt}}c@{\hspace{0pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{0pt}}         
 %
        }
        \hline\hline
        \multicolumn{1}{c}{$\mathcal{K}$} && \multicolumn{2}{c}{\GMop}   && \multicolumn{2}{c}{\GMtan}   && \multicolumn{2}{c}{\GMavg}   && \multicolumn{2}{c}{\GMprob} \\
                                   %& \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
        \cline{1-1} \cline{3-4}                 \cline{6-7}                 \cline{9-10}                  \cline{12-13}
        ~~\SDS && \IID & \coSim && \orderI & \orderII && \IID & \coSim && \IID & \coSim \\

        \hline
acc  &&  0.844 		&  0.854          &&  0.836 &  0.841 &&  0.838 &  0.837 	 &&  - & -  \\
pre  &&  \textbf{0.917} &  0.914          &&  0.892 &  0.889 &&  0.905 &  0.861          &&  - & -  \\
rec  &&  0.757          &  0.782 	  &&  0.764 &  0.781 &&  0.756 &  \textbf{0.804} &&  - & -  \\
F1   &&  0.829          &  \textbf{0.843} &&  0.823 &  0.831 &&  0.824 &  0.832          &&  - & -  \\
AUC  &&  0.919		&  \textbf{0.932} &&  0.923 &  0.925  && 0.918 & 0.917  	 &&  - & -  \\



%        \hline\hline
%	& \multicolumn{2}{c}{\GMop}   && \multicolumn{2}{c}{\GMtan}   && \multicolumn{2}{c}{\GMavg}   && \multicolumn{2}{c}{\GMprob} \\
%				   %& \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
%\cline{2-3}                 \cline{5-6}                 \cline{8-9}                  \cline{11-12}
%	& \IID & \coSim && \orderI & \orderII && \IID & \coSim && \orderI & \orderII \\
%	\hline
%Acc & 0.888 & \textbf{0.894}  && 0.870 & 0.881	&& 0.883               & 0.877                && 0.807 & 0.820  \\
%Pre & 0.942 & 0.939           && 0.933 & 0.934	&& \textbf{0.944}      & 0.904                && 0.842 & 0.834  \\
%Rec & 0.826 & 0.842           && 0.797 & 0.820	&& 0.815               & \textbf{0.843}       && 0.757 & 0.805  \\
%F1  & 0.880 & \textbf{0.888}  && 0.860 & 0.873	&& 0.875               & 0.873                && 0.797 & 0.819  \\
%AUC & 0.947 & \textbf{0.957}  && 0.953 & 0.955	&& 0.948               & 0.942                && 0.894 & 0.901  \\

        \hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
       In this table, ``acc'', ``pre'', ``rec'' and ``AUC'' represent
        accuracy, precision, recall, and the area under an receiver operating characteristic curve, respectively.
        In \GMtan, ``\orderI'' is the kernel, in which the similarity between two drug combinations is calculated by the feature vectors, whose dimensions correspond to only one drug.
        As for ``\orderII'', the similarity between two drug combinations is calculated by the feature vectors, which have dimensions that correspond to different pairs of drugs.


          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
 %  \end{center}	
  \end{threeparttable}
\end{table}
%


==> results_table/results_AD_2000.tex <==
\begin{table}[t]
  \centering
  \caption{Overall Performance Comparison of \Dtwok}
  \label{table:result_2k}
  \begin{threeparttable}
   %\begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{0pt}}l@{\hspace{3pt}}
          @{\hspace{0pt}}c@{\hspace{0pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{3pt}}
          @{\hspace{3pt}}c@{\hspace{0pt}}
          %
        }
        \hline\hline
        \multicolumn{1}{c}{$\mathcal{K}$} && \multicolumn{2}{c}{\GMop}   && \multicolumn{2}{c}{\GMtan}   && \multicolumn{2}{c}{\GMavg}   && \multicolumn{2}{c}{\GMprob} \\
                                   %& \multicolumn{2}{c}{\GMgd} && \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
        \cline{1-1} \cline{3-4}                 \cline{6-7}                 \cline{9-10}                  \cline{12-13}
        ~~\SDS && \IID & \coSim && \orderI & \orderII && \IID & \coSim && \IID & \coSim \\

        \hline

acc  &&  0.929 & \textbf{0.938}&& 0.897 & 0.910 && 0.924 & 0.912 && 0.845 & 0.860  \\
pre  &&  0.954 & \textbf{0.959}&& 0.941 & 0.942 && 0.957 & 0.917 && 0.839 & 0.860  \\
rec  &&  0.902 & \textbf{0.916}&& 0.847 & 0.873 && 0.888 & 0.907 && 0.854 & 0.869  \\
F1   &&  0.927 & \textbf{0.937}&& 0.891 & 0.906 && 0.921 & 0.912 && 0.846 & 0.861  \\
AUC  &&  0.973 & \textbf{0.976}&& 0.964 & 0.968 && 0.970 & 0.960 && 0.920 & 0.926  \\


%        \hline\hline
%	 & \multicolumn{2}{c}{\GMop}	&& \multicolumn{2}{c}{\GMtan}	&& \multicolumn{2}{c}{\GMavg}	&& \multicolumn{2}{c}{\GMprob} \\
%				  %& \multicolumn{2}{c}{\GMop} && \multicolumn{2}{c}{\GMavg} && \multicolumn{2}{c}{\GMprob} && \multicolumn{2}{c}{\GMtan} \\
%				     \cline{2-3}		 \cline{5-6} 		     \cline{8-9}		  \cline{11-12}
%	& \IID       & \coSim        && \orderI & \orderII	&& \IID & \coSim	&& \IID & \coSim	\\
%	\hline
%Acc       & 0.929 & \textbf{0.938}&& 0.897 & 0.910 && 0.924 & 0.912 && 0.845 & 0.860  \\
%Pre       & 0.954 & \textbf{0.959}&& 0.941 & 0.942 && 0.957 & 0.917 && 0.839 & 0.860  \\
%Rec       & 0.902 & \textbf{0.916}&& 0.847 & 0.873 && 0.888 & 0.907 && 0.854 & 0.869  \\
%F1        & 0.927 & \textbf{0.937}&& 0.891 & 0.906 && 0.921 & 0.912 && 0.847 & 0.864  \\
%AUC       & 0.973 & \textbf{0.976}&& 0.964 & 0.968 && 0.970 & 0.960 && 0.920 & 0.926  \\
	
	\hline
        \hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
In this table, ``acc'', ``pre'', ``rec'' and ``AUC'' represent
        accuracy, precision, recall, and the area under an receiver operating characteristic curve, respectively.
        In \GMtan, ``\orderI'' is the kernel, in which the similarity between two drug combinations is calculated by the feature vectors, whose dimensions correspond to only one drug.
        As for ``\orderII'', the similarity between two drug combinations is calculated by the feature vectors, which have dimensions that correspond to different pairs of drugs.

          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%


==> results_table/temp.tex <==
\begin{table}[t]
  \centering
  \caption{ Average Percentage of \Dscider Drugs}
  \label{table:enrich}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
%	{p{25mm}|p{10mm}|p{10mm}|p{10mm}
	@{\hspace{0pt}}c@{\hspace{10pt}}
	@{\hspace{8pt}}c@{\hspace{8pt}}   
	@{\hspace{8pt}}c@{\hspace{8pt}}       
	@{\hspace{8pt}}c@{\hspace{8pt}}
	%@{\hspace{8pt}}c@{\hspace{0pt}}
	%@{\hspace{8pt}}c@{\hspace{8pt}}
        %@{\hspace{8pt}}c@{\hspace{0pt}}
	%@{\hspace{8pt}}c@{\hspace{0pt}}
	%@{\hspace{8pt}}c@{\hspace{0pt}}
	}
        \hline\hline
		\Mmist	& \Mmis		 & \Mpos 	&\Mt \\
			%& $\mathcal{D}^{{2000}}$ & $\mathcal{D}^{{4000}}$	& $\mathcal{D}^{{6948}}$	\\
        \hline
	  % 0.1333	 &0.1662 &0.2425 &0.8983\\
	   13.3 & 16.6&24.2&89.8 \\
	\hline\hline
		\Nmist  &\Nmis & \Nneg &\Nt \\
	\hline
	%0.3071       &   0.1856      &  0.1557  & 0.1000\\
	 30.7&18.5&15.5&0.10 \\

	%Top-10  miss   & 0.1742  & 0.3095   &	0.3071 \\	
	%Top-all miss   & 0.1671  & 0.1830   &   0.1856	\\	
	%All negative   & 0.1412  & 0.1513   &   0.1557	\\	
	%All positive   & 0.2080	 & 0.2510   &	0.2425 \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  \textcolor{red}{
	  For each drug combination, the percentage is calculated by 
	  the number of drugs, which can cause myopathy on its own (i.e., drugs in \Dscider), divided by the drug combination order.}
	  \Mpos and \Nneg represent the sets of drug combinations, whose labels are all positive and negative, respectively.
	  \Mmis and \Nmis are the sets of all misclassified drug combinations in \Mpos and \Nneg , respectively.
	  \Mmist  is the set of misclassified drug combinations in \Mmis with the top-10 lowest negative prediction values and 
	  \Nmist is the set of misclassified drug combinations in \Nmis with the top-10 highest positive prediction values.
	  \Mt and \Nt are the sets of correctly classified drug combinations in \Mpos and \Nneg with the top-10 highest and lowest prediction values, respectively.
	  	
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}
%


==> results_table/temp_top_prediction_combinations_D4000.tex <==
\begin{table*}[!h]
  \centering
  \caption{ top prediction value combinations in \GMop of \DIVk  }
  \label{table:top_com_d4k}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{10mm}|p{100mm}
        @{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{8pt}}l@{\hspace{8pt}}
	}
        \hline\hline
		N	& prd	& frq &OR & Combinations		\\
        \hline


1 &4.291 & 3  &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
2 &3.954 & -  & 140.9700&\textbf{atorvastatin} \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin} tadalafil  \\
3 &3.948 & -  & 52.0340 &\textbf{atorvastatin} \textbf{fenofibrate} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
4 &3.881 & -  & 83.2800 &\textbf{atorvastatin} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
5 &3.797 & -  & 18.8940 &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{rosuvastatin} \textbf{simvastatin}  \\
6 &3.726 & 10 &  -      &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{fenofibrate} \textbf{rosuvastatin}  \\
7 &3.557 & 9  &  -      &\textbf{atorvastatin} \textbf{fenofibrate} \textbf{pravastatin} \textbf{simvastatin}  \\
8 &3.518 & 11 &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{simvastatin}  \\
9 &3.496 & -  & 11.6710 &\textbf{atorvastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
10&3.422 & 6  &  -      &\textbf{atorvastatin} celecoxib escitalopram gabapentin levofloxacin levothyroxine liothyronine risedronate \textbf{simvastatin}  \\

        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  Prediction values, frequency and odds ratio are denoted as prd, frq and OR, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/temp_top_prediction_combinations_D6928.tex <==
\begin{table*}[!h]
  \centering
  \caption{Top classified myopathy-inducing drug combinations from \GMop with \SDSc} 
  \label{table:top_com_d6k}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{10mm}|p{100mm}
        @{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{8pt}}l@{\hspace{8pt}}
	}
        \hline\hline
	N       & prd   & frq &\OR & Combinations                \\
        \hline
1 &4.167 & 3  &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
2 &4.009 & -  & 11.372  &\textbf{atorvastatin} \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
3 &3.776 & -  & 50.043  &\textbf{atorvastatin} \textbf{fenofibrate} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
4 &3.734 & -  & 68.232  &\textbf{atorvastatin} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
5 &3.676 & -  & 45.487  &\textbf{atorvastatin} \textbf{lovastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
6 &3.618 & -  & 136.470 &\textbf{atorvastatin} \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin} tadalafil  \\
7 &3.573 & 9  &  -      &\textbf{atorvastatin} \textbf{fenofibrate} \textbf{pravastatin} \textbf{simvastatin}  \\
8 &3.552 & 10 &  -      &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{fenofibrate} \textbf{rosuvastatin}  \\
9 &3.519 & -  & 22.746  &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{rosuvastatin} \textbf{simvastatin}  \\
10&3.461 & 11 &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{simvastatin}  \\


        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
In this table, ``prd'', ``frq'' and ``\OR'' represent prediction values, frequency and odds ratio, respectively.
          Drugs in \Dscider are marked in \textbf{bold}.

	%Prediction values, frequency and odds ratio are denoted as ``prd'', ``frq'' and ``\OR'', respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/temp_top_prediction_combinations_D6928_miss_classi.tex <==
\begin{table*}[t!]
  \centering
  \caption{Misclassified non-myopathy-inducing drug combinations from \GMop with \SDSc}
  \label{table:top_com_d6k_miss}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
 	@{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	}
        \hline\hline
N       & prd &frq &\OR     & combinations          \\
        \hline
        1&2.696 & 26 & -       &\textbf{atorvastatin} \textbf{fenofibrate} rosiglitazone \textbf{simvastatin}  \\
        2&2.507 & 26 & -       &\textbf{allopurinol} amlodipine \textbf{atorvastatin} levothyroxine naproxen omeprazole \textbf{simvastatin}  \\
        3&1.878 & 22 & -       &acetylsalicylicacid \textbf{atorvastatin} bisoprolol clopidogrel ramipril \textbf{simvastatin}  \\
        4&1.855 & 27 & -       &acetylsalicylicacid atenolol \textbf{atorvastatin} furosemide lansoprazole lisinopril nitroglycerin  \\
        5&1.785 & 21 & -       &\textbf{citalopram} clozapine isosorbidemononitrate prochlorperazine \textbf{simvastatin} \textbf{zopiclone}  \\
        6&1.750 & - & 0.842    &amlodipine bisoprolol \textbf{pravastatin} ramipril \textbf{simvastatin} spironolactone warfarin  \\
        7&1.696 & 22 & -       &amlodipine clopidogrel ibuprofen omeprazole ramipril \textbf{simvastatin}  \\
        8&1.669 & 29 & -       &bisoprolol flecainide ramipril \textbf{simvastatin}  \\
        9&1.613 & 35 & -       &\textbf{aripiprazole} \textbf{atorvastatin} bendroflumethiazide clozapine diazepam folicacid furosemide iron lactulose lansoprazole perindopril ramipril trimethoprim \textbf{zopiclone}  \\
        10&1.549& - & 0.875    &lansoprazole omeprazole pantoprazole rabeprazole  \\
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	 In this table,  ``prd'', ``frq'' and ``\OR'' represent prediction values, frequency and odds ratio, respectively.
	Drugs in \Dscider are marked in \textbf{bold}.  
	\hl{Prediction values, frequency and odds ratio are denoted as ``prd'', ``frq'' and ``\OR'', respectively.}
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/top_prediction_combinations_D2000.tex <==
\begin{table*}[!h]
  \centering
  \caption{top prediction value combinations in \GMop of \DIIk }
  \label{table:top_com_d2k}
  \vspace{-10pt}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{100mm}
	@{\hspace{0pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}   
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{3pt}}l@{\hspace{pt}}
	}
        \hline\hline
	N	& prd &frq	& Combinations		\\
        \hline
1 &3.064 & 3 &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}   \\
2 &2.784 & 9 &\textbf{atorvastatin} \textbf{fenofibrate} \textbf{pravastatin} \textbf{simvastatin}   \\
3 &2.755 & 5 &\textbf{atorvastatin} fluconazole levothyroxine \textbf{simvastatin}   \\
4 &2.747 & 11&\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{simvastatin}   \\
5 &2.602 & 6 &\textbf{atorvastatin} celecoxib escitalopram gabapentin levofloxacin levothyroxine liothyronine risedronate \textbf{simvastatin}   \\
6 &2.528 & 4 &alprazolam \textbf{atorvastatin} imipramine levothyroxine \textbf{simvastatin}   \\
7 &2.504 & 6 &\textbf{atorvastatin} fexofenadine fluticasonepropionate levofloxacin nitrofurantoin \textbf{simvastatin}   \\
8 &2.452 & 4 &\textbf{allopurinol} \textbf{amiodarone} \textbf{atorvastatin} furosemide omeprazole \textbf{simvastatin}   \\
9 &2.420 & 13&\textbf{atorvastatin} esomeprazole hydrochlorothiazide losartan potassium ramipril \textbf{simvastatin}   \\
10&2.416 & 5 &acetylsalicylicacid lansoprazole lisinopril \textbf{pravastatin} quinine \textbf{simvastatin}   \\
		

	
        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	 Prediction values and frequency are denoted as prd and frq, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/top_prediction_combinations_D4000.tex <==
\begin{table*}[h!]
  \centering
  \caption{ top prediction value combinations in \GMop of \DIVk  }
  \label{table:top_com_d4k}
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	%{p{10mm}|p{10mm}|p{15mm}|p{10mm}|p{100mm}
        @{\hspace{0pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
	@{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}r@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.8\linewidth}@{\hspace{0pt}}
	%@{\hspace{8pt}}l@{\hspace{8pt}}
	}
        \hline\hline
		N	& prd	& frq &OR & Combinations		\\
        \hline


1 &4.291 & 3  &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
2 &3.954 & -  & 140.9700&\textbf{atorvastatin} \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin} tadalafil  \\
3 &3.948 & -  & 52.0340 &\textbf{atorvastatin} \textbf{fenofibrate} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
4 &3.881 & -  & 83.2800 &\textbf{atorvastatin} metformin \textbf{pravastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
5 &3.797 & -  & 18.8940 &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{rosuvastatin} \textbf{simvastatin}  \\
6 &3.726 & 10 &  -      &\textbf{atorvastatin} \textbf{ezetimibe} \textbf{fenofibrate} \textbf{rosuvastatin}  \\
7 &3.557 & 9  &  -      &\textbf{atorvastatin} \textbf{fenofibrate} \textbf{pravastatin} \textbf{simvastatin}  \\
8 &3.518 & 11 &  -      &\textbf{atorvastatin} lansoprazole \textbf{pravastatin} \textbf{simvastatin}  \\
9 &3.496 & -  & 11.6710 &\textbf{atorvastatin} \textbf{rosuvastatin} \textbf{simvastatin}  \\
10&3.422 & 6  &  -      &\textbf{atorvastatin} celecoxib escitalopram gabapentin levofloxacin levothyroxine liothyronine risedronate \textbf{simvastatin}  \\

        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  Prediction values, frequency and odds ratio are denoted as prd, frq and OR, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table*}
%


==> results_table/whole_freqs_average_info.tex <==
\begin{table}[!h]
  \caption{Statistical Information of \Dall }
  \label{table:Statis_whole}
  \centering
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
	@{\hspace{2pt}}l@{\hspace{10pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}          
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	@{\hspace{2pt}}r@{\hspace{2pt}}
	}
        \hline\hline
				& \AALL	& \BALL	& \CALL        & \DALL \\
        \hline
	average order		& 6.1002		& 2.3505        	& 3.5882     		& 7.0961		\\
	average freqency	& 1.7607		& 225.3172      	& 13.7295               & 1.4022		\\
	average OR 		& -	        	& 0.5460		& 16.3432               & -	 		\\


        \hline\hline
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	  There are 621,449 different drug combinations and they are denoted as \AALL.
	  There are 27,387 different drug combinations and they are denoted as  \DALL.
	  %There are 10,250 different sets of drugs both in control and case events.
          In these 10,250 drug combinations, there are 8,986 of them whose \OR values are larger than one and they are denoted as \CALL.
	  In these 10,250 drug combinations, there are 1,264 of them whose \OR values are smaller than one and they are denoted as \BALL.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}
%

